Accessibility Issues in Ad-Driven Web Applications

Website accessibility is essential for inclusiveness and regulatory compliance. Although third-party advertisements (ads) are a vital revenue source for free web services, they introduce significant accessibility challenges. Leasing a website\'s space to ad-serving technologies like DoubleClick results in developers losing control over ad content accessibility. Even on highly accessible websites, third-party ads can undermine adherence to Web Content Accessibility Guidelines (WCAG). We conduct the first large-scale investigation of 430K website elements, including nearly 100K ad elements, to understand the accessibility of ads on websites. We seek to understand the prevalence of inaccessible ads and their overall impact on the accessibility of websites. Our findings show that 67% of websites experience increased accessibility violations due to ads, with common violations including Focus Visible and On Input. Popular ad-serving technologies like Taboola, DoubleClick, and RevContent often serve ads that fail to comply with WCAG standards. Even when ads are WCAG compliant, 27% of them have alternative text in ad images that misrepresents information, potentially deceiving users. Manual inspection of a sample of these misleading ads revealed that user-identifiable data is collected on 94% of websites through interactions, such as hovering or pressing enter. Since users with disabilities often rely on tools like screen readers that require hover events to access website content, they have no choice but to compromise their privacy in order to navigate website ads. Based on our findings, we further dissect the root cause of these violations and provide design guidelines to both website developers and ad-serving technologies to achieve WCAG-compliant ad integration.

==> ICSE/parts/abstract.tex <==
\begin{abstract}
Website accessibility is essential for inclusiveness and regulatory compliance. Although third-party advertisements (ads) are a vital revenue source for free web services, they introduce significant accessibility challenges. Leasing a website's space to ad-serving technologies like DoubleClick results in developers losing control over ad content accessibility. Even on highly accessible websites, third-party ads can undermine adherence to Web Content Accessibility Guidelines (WCAG).
%, especially for visually impaired users who cannot distinguish original content from ads, increasing the risk of exploitation such as phishing and scams. Therefore, developers must address the accessibility impact of ads during web development.
We conduct the first-of-its-kind large-scale investigation of 430K website elements, including nearly 100K ad elements, to understand the accessibility of ads on websites. 
% 
We seek to understand the prevalence of inaccessible ads and their overall impact on the accessibility of websites.
% 
Our findings show that 67\% of websites experience increased accessibility violations due to ads, with common violations including Focus Visible (WCAG 2.4.7), and On Input (WCAG 3.2.2). 
% 
Popular ad-serving technologies like Taboola, DoubleClick, and RevContent often serve ads that fail to comply with WCAG standards. 
% 
Even when ads are WCAG compliant, 27\% of them have alternative text in ad images that misrepresents information, potentially deceiving users. 
% 
Manual inspection of a sample of these misleading ads revealed that user-identifiable data is collected on 94\% of websites through interactions, such as hovering or pressing enter.
% Further assessment of the privacy risk of ads reveals that interacting with ads through hovering and pressing enter resulted in the collection of user-identifiable data on 94\% of the websites. 
% 
Since users with disabilities often rely on tools like screen readers that require hover events to access website content, they have no choice but to compromise their privacy in order to navigate website ads. 
% 
Based on our findings, we further dissect the root cause of these violations and provide design guidelines to both website developers and ad-serving technologies to achieve WCAG-compliant ad integration.

% Our manual inspection of 50 websites revealed that






% Our findings show that 67\% of websites experience a notable increase in accessibility violations due to advertisements.
% The most common types of violations in advertisements include Focus Visible (WCAG 2.4.7), On Input (WCAG 3.2.2), and In Context (WCAG 2.4.4). 
% Additionally, we demonstrate that many popular ad-serving technologies, such as DoubleClick, Taboola, and Facebook, often fail to comply with WCAG standards for websites.
% Even when an ad is WCAG-compliant, we find that 27\% of the alt text in ad images misrepresents information, potentially deceiving users. 
% 
% 

% 



% Web accessibility is crucial for maintaining inclusiveness and meeting regulatory requirements.  
% % 
% While third-party advertisements (ads) are a key source of revenue for free web services, they pose significant accessibility challenges. 
% % 
% By leasing digital space on websites to ad-serving technologies like DoubleClick, developers forfeit control over the accessibility of ad content. 
% % 
% Inaccessible third-party ads may compromise website accessibility.  visually impaired users' ability to differentiate original content from ads. 
% %This increases the risk of exploitation, including phishing and scams. 
% % 
% Therefore, web developers must ensure that standards for websites, specifically the WCAG guidelines, during web development.


%Web accessibility is crucial for digital inclusivity and regulatory compliance. Third-party advertisements, while key for revenue in free web services, pose accessibility challenges. When developers use ad-serving technologies like DoubleClick, they lose control over ad content accessibility. This can undermine even ADA-compliant webpages, especially for visually impaired users relying on screen readers to navigate content. The inability to distinguish ads from original content increases vulnerability to phishing and scams. Developers must therefore consider and address the impact of ads on accessibility during web development.

% Free and open internet relies on third-party advertisements on websites to generate revenue. 
% % 
% By leasing digital space to ad-serving technologies like DoubleClick, developers lose control over the accessibility of ad content.
% % 
% Even if a webpage is ADA-compliant, third-party ads can undermine its accessibility, particularly for visually impaired users who cannot distinguish original content from ads when using assistive technologies like screen readers. 
% % 
% This increases the risk of exploitation, including phishing and scams. %In the US, over 84 million people have disabilities, yet a significant space on web pages is still not accessible to users without impairments. 
% % 
% Making web applications accessible is crucial for maintaining inclusiveness and is often a regulatory requirement. Therefore, during web development, developers must understand and address the accessibility impact of serving ads on their web pages.
% %

% We conduct the first large-scale, in-depth investigation to understand the accessibility of web advertisements from a web developer's perspective. 
% % 
% Our findings show that website advertisements increase accessibility violations by X\%.
% % 
% The most common types of violations in advertisements include X, Y, and Z. 
% % 
% We also demonstrate that many popular ad-serving technologies often fail to comply with ADA standards. 
% % 
% Even when an Ad is ADA-compliant, we find that 27\% of the alt-text in ad images misrepresents information, deceiving users.
% % 
% Assistive technologies like screen readers utilize {\tt onhover} events to let users access web content. We manually inspected 50 websites by interacting with misleading ads through hovering and clicking and found that X\% collected user-identifiable data. Thus, users with disabilities have no choice but to compromise their privacy in order to navigate the web.
% % 
% The findings of this work highlight the limitations of existing tools in measuring the true accessibility of the webpage and the precautions that web developers need to take when incorporating ads in webpages. 


%of leasing digital space to ad-serving technologies that comply with accessibility standards and encourage these technologies to improve the accessibility of their ads.

% Gulzar's abstract
% The free and open internet thrives by hosting third-party content, such as ads, that enable developers to earn revenue. To host an advertisement, web developers lease digital space on their web pages to ad agencies, such as Google and Taboola, who then serve advertisements on that space when a user visits the webpage. Inadvertently, web developers give up control of the web page's component serving ads and, therefore, are unable to verify the accessibility of significant content on their webpage. Even when the originally developed webpage claims to be ADA-compliant and accessible, the third-party inaccessible ads can severely harm the accessibility of the web page when served to the user. This is especially problematic because visually impaired users cannot distinguish organic content from advertisements, which is more likely to lead to exploitation, including phishing, fraud, and scams. In the US alone, over 84 million individuals live with some form of disability, yet modern webpages primarily cater to users without impairments.

% We conducted the first large-scale, in-depth investigation of 5,000 websites to understand the accessibility of web advertisements through the lens of a web developer. Using state-of-the-art, code-level content-blocking techniques, we measured the impact of advertisements on website accessibility and how exactly they deteriorate the browsing experience for visually impaired users. By combining investigations on ad accessibility issues with tracing web advertisements to their ad-serving agency, we identified the ad-serving technologies that most frequently deteriorate the accessibility of webpages. Users with disabilities rely on assistive technologies like screen readers to navigate web pages. A critical issue is the lack of proper labeling for third-party content. If an advertisement is accessible via alternate text, we used a large language model to verify if the alternate description of the ad truly conveys its intent as well as the content of the ad image. Our investigation reveals that web advertisements increase accessibility violations by 12\%, where more than half of the X number of ads are completely invisible to users with visual impairments. Among the ads with alternate descriptions, nearly 27\% of those have misrepresented alternate text, misleading users into interacting with ads that may violate their privacy.

% The free and open internet thrives by hosting third-party content, such as ads, that enable developers to earn revenue. To host an advertisement, web developers lease digital space on their web pages to ad agencies, such as Google and Taboola, who then serve advertisements on that space when a user visits the webpage. Inadvertently, web developers give up control of the web page's component serving ads and, therefore, are unable to verify the accessibility of significant content on their webpage. Even when the originally developed webpage claims to be ADA-compliant and accessible, the third-party inaccessible ads can severely harm the accessibility of the web page when served to the user. This is especially problematic because visually impaired users cannot distinguish organic content from advertisements, which is more likely to lead to exploitation, including phishing, fraud, and scams.  In the US alone, over 84 million individuals live with some form of disability, yet modern webpages primarily cater to users without impairments. 

% We performed the first large-scale, in-depth investigation of 5,000 websites to understand the accessibility of web advertisement through the lens of a web developer. Using state-of-the-art, code-level content-blocking techniques, we measured the impact of advertisements on website accessibility and how exactly they deteriorate the browsing experience for visually impaired users.   By combining investigations on ad accessibility issues with tracing web advertisements to its ad-serving agency, we identify the ad-serving technologies that most frequently deteriorate the accessibility of webpages. Users with disabilities rely on assistive technologies like screen readers to navigate web pages. A critical issue is the lack of proper labeling for third-party content.  If an advertisement is accessible via alternate text, we use the large language model to verify if the alternate description of the ad truly converts its intent as well as the content of the ad image.  Our investigation reveals that web advertisements increase accessibility violations by 12\%, where more than half of the X number of ads are completely invisible to users with visual impairments. Among the ads with alternate descriptions, nearly 27\% of those have misrepresented alternate text, misleading users into interacting with ads that may violate their privacy.


\end{abstract}


==> ICSE/parts/background.tex <==
\begin{figure}[!t]
% \vspace{0.1in}
\begin{subfigure}{.23\textwidth}
    \fbox{\includegraphics[width=.99\linewidth, height=2.6cm]{images/ad-issues-sample.png}}
    \caption{Accessibility Violations in Ad Slots of Taboola.}
\end{subfigure}
\hspace{.05in}
\begin{subfigure}{.23\textwidth}
    \fbox{\includegraphics[width=.99\linewidth]{images/ad-screenreader.png}}
    \caption{Ads are not accessible to users relying on screen readers.}
\end{subfigure}
\caption{Violation identified in Taboola ad slots and its impact on how screen reader users experience the website.} 
\vspace{-4ex}
\label{fig:ad-issues-sample}
\end{figure} 
\begin{figure*}[h]
    \centering
      \includegraphics[width=0.9\textwidth]{images/overview.png}
      %  \put(-392,5){{\ding{202}}}
      %  \put(-316,5){{\ding{203}}}
      % \put(-250,5){{\ding{204}}}
      % \put(-193,5){{\ding{205}}}
      % \put(-126,5){{\ding{206}}}
      % \put(-9,5){{\ding{207}}}
        \caption{Overview of our methodology involving generating accessibility reports for each website with (\rwa) and without ads (\rwoa), then comparing them to isolate and analyze the accessibility violations caused by only ads ($R_{ads-only}$).}
        \label{fig:overview}
        \vspace{-.2in}
\end{figure*}
\section{Motivating Example}
\label{sec:motivation}
% 
This section presents a case study showing how some ads on websites violate accessibility guidelines and affect the overall website's accessibility.
%can deteriorate the accessibility of the website. 
Alaska's News Source, {\tt alaskasnewssource.com}\cite{alaskanews}, provides local news, weather updates, sports coverage, and community events for the state of Alaska.
%
It is ranked 14\textsuperscript{th} in the top 5K in the news and media category.
% 
In the stock Chrome browser, this website shows numerous ads in ad slots—three at the top and one at the bottom, as seen in Figure \ref{fig:motivating-example}(a). 
% 
The top slots are served by Taboola\cite{Taboola} and the bottom by Google Ads\cite{Google-ads}.
% When loaded in the stock chrome browser, this website contains numerous advertisements placed in ad slots---three ads in the top slot and one ad on the bottom slot---as seen in Figure \ref{fig:motivating-example}(a). 
% % 
% These ad slots are filled by two different ad-serving technologies. Taboola\cite{Taboola} serves the top-one slots, and Google Ads\cite{Google-ads} serves those on the bottom.


\noindent\textbf{Website accessibility without ads.} 
In the first step, we generate the accessibility report for {\tt alaskasnewssource.com} by computing the violation count without including any ads.
% 
We remove ads from the website to emulate the website development stage, where website developers are unaware of the precise ads that will be served by the ad-serving technologies. 
% 
This is a common practice employed by many website quality and accessibility checkers like Google Lighthouse \cite{Google-lighthouse} that do not include ads in their accessibility evaluations. 
% 
We use IBM's accessibility checker chrome extension, a tool used by over 20K developers\cite{IBM-accessibility}, mainly because it evaluates all website elements, including ad elements. 
% 
To remove ads from the website, we deploy the uBlock Origin's Chrome extension, which has over 700K users\cite{uBlock-origin}, to block all ads on the website.  
%
As seen in Figure \ref{fig:motivating-example}(b), all ads on {\tt alaskasnewssource.com} are removed, and the accessibility checker reports 126 violations.
% 
For example, the element in Listing \ref{lst:motivation} violates the WCAG 2.4.4 (Link Purpose) \cite{WCAG-list} guideline because it lacks descriptive link text, label, or an image with a text alternative. 
% 
The guideline requires that links must have a clear purpose that users can understand, especially when the link is not accompanied by any other textual context. 
% 
This can be resolved by adding {\tt aria-label="Download the Alaska's News Source Streaming Apps"} to this tag by developer. 
% 
\lstdefinestyle{base}{
language=html,
moredelim=**[is][\color{red}]{@}{@},
moredelim=**[is][\color{darkgreen}]{~}{~},
numbers=left,
numberstyle=\tiny,
stepnumber=1,
numbersep=5pt,
escapechar=`
}
\begin{lstlisting}[caption={Anchor tag missing descriptive text},language=html, label={lst:motivation}, style=base]
<a data-tb-link="" target="\_self" rel="" href="https://www.alaskasnewssource.com/page/how-to-download-the-alaskas-news-source-streaming-apps/" class="link | text-reset d-block h-100 w-100">
\end{lstlisting}
% 
Most accessibility violations can easily be addressed by the developer with simple refactoring of the website's code (\ie HTML, CSS, and JS). 

\noindent\textbf{Website accessibility with ads.} Next, we compute accessibility report for {\tt alaskasnewssource.com} by computing the violation count with ads, as displayed to the user.
% 
This setting allows us to demonstrate the increase in the violations attributed to ads on the website.

% 
Figure \ref{fig:motivating-example}(c) shows that ads appear on the website as they did on a normal visit. 
% ((Second Value – First Value) ÷ First Value) x 100%
The accessibility checker reports 279 violations, showing a 121.4\% change in the violation count. 
% 
Given that the only difference between the two websites is the presence of ads, it is reasonable to attribute the increase in accessibility violations to the ads.
% 
We further examine specific violations related to ads, particularly concerning the ad slots Taboola serves. 
% 

Figure \ref{fig:ad-issues-sample}(a) shows violations identified by the accessibility checker across three ad slots for Taboola (highlighted with a red circle around their title and short description).
% 
This violates the WCAG 2.1.1 (Keyboard) guideline\cite{WCAG-list} because the element cannot be interacted with using a keyboard alone.
% 
All ad images are designed with a {\tt link role}, which does not include a tabbable element. 
% 
Thus, users who rely on keyboard navigation cannot directly access these elements. 
% 
Additionally, most of these ad images do not include alternate text to make them accessible for visually impaired users.   
% 
We further test the accessibility of these ads with  Google's Chrome Vox screen reader\cite{Chrome-vox}.
% 
Vox only announces {\tt image for Taboola advertising unit} on tab focus without reading the title and short description of each ad. 
% 
Figure \ref{fig:ad-issues-sample}(b) shows how the website and ads appear to visually impaired users using screen readers, leaving ads' content mostly inaccessible except the two vague alternate texts.
%


\textbf{\textit{It is difficult for a website developer to anticipate and address ad accessibility violations as these violations are non-deterministic and occur after the deployment of the website. }} 
% 
In the case of {\tt alaskasnewssource.com}, ads are negatively impacting accessibility, which raises the concern of whether such an effect is prevalent across all ads: (1) if yes, then what kinds of violations do they cause? and (2) if not, then does the accessible information in these ads adequately represent their content? Similarly, it is useful to know which ad-serving technologies are serving more inaccessible ads.


==> ICSE/parts/citations.tex <==
\begin{thebibliography}{00}

\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.









\end{thebibliography}

==> ICSE/parts/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}
\label{sec:conclusion}

Website ads are an integral part of a website and are essential for supporting free Internet; however, they often fail to meet basic accessibility standards.
This paper presents the first extensive study on the accessibility issues of website ads. Our research reveals that 67\% of websites show a noticeable increase in accessibility violations due to ads. We also discovered that popular ad-serving technologies do not adhere to the WCAG guidelines when displaying ads, and nearly one-quarter of ads that do comply with WCAG guidelines have misleading alt text.
Our findings provide insight into the challenges faced by website developers in integrating ads while maintaining accessibility. This research suggests ways for developers to enforce accessibility standards to lessen the impact of ads on overall website's accessibility.

==> ICSE/parts/discussion.tex <==
\section{Discussion and Takeaways}
\label{sec:discussion}
% 
Based on our empirical investigation, we provides insights for website developers and ad-serving technologies to address ad accessibility violations and highlights future research avenues for improving the website experience for users with disabilities.
% Based on our empirical investigation, we draw insights and takeaways for web developers and ad-serving technologies to help address accessibility issues in web ads.
% We also discover avenues for future research on developer tools to make the internet more inclusive and accessible and improve the web experience for users with disabilities. 

%%
\noindent\textbf{Accessibility-promoting ad integration for website developers.}
Ad integration is crucial for ad-driven websites. Developers must ensure high accessibility and WCAG compliance, which can be a regulatory requirement\cite{WCAG-21}. Once published, the developer cannot modify the website to address ad-related accessibility issues since new ads may introduce different violations. Developers can ensure two key aspects to improve ad accessibility during integration.
% Ad integration is a critical step in the development of ad-driven websites. When the website serves ads, it is the responsibility of the website developer to ensure high accessibility and WCAG compliance, which, in certain cases, is a regulatory requirement\cite{WCAG-21}. Once an ad slot is placed on the website and the website is published, the developer cannot modify or refractor the website's code to improve ad-related accessibility issues since each visit to the website brings a new ad, which may encounter a different accessibility violation. Website developers can ensure two key things to improve ad accessibility during ad integration.
% 
First, they can inject JavaScript to enforce CSS rules (using {\tt !important}) to implement basic checks on WCAG Type A violations. 
% 
For instance, a script can be added to ensure all text elements have sufficient color contrast. Such a script can be triggered on {\tt onload} events to detect certain accessibility violations and address them appropriately, if possible.  
% 
Some Type AA violations can also be addressed by injecting similar checks in the JavaScript, such as ensuring all interactive elements are keyboard accessible.
% 
Secondly, developers can run accessibility checks on their websites post-deployment (similar to our analysis) to analyze ad elements and derive specific self-correcting strategies to address those concerns.


%and address any remaining accessibility issues.
% \gulzar{1. Why ads are inaccessible? is it advertiser or publisher or web developer? 2.  automated accessibility enhancing  tools exist, but they only work on the developer side and at the client side; the violation will be different for every load. Anticipating accessibly for ads is hard. }
%%
\noindent\textbf{Accessibility strategies for ad-serving technologies.}
Website developers integrate ads on their websites by leasing ad space to ad-serving technologies. 
% 
These ad-serving technologies often enroll in programs such as the Acceptable Ads program \cite{Acceptable-ads} and adhere to guidelines set by the Interactive Advertising Bureau (IAB) \cite{IAB}.
% 
The Acceptable Ads Program promotes non-intrusive ad formats that respect user experience, requiring adherence to specific display guidelines. 
% 
The IAB sets comprehensive standards for digital advertising, including ad formats, measurement, and data privacy, ensuring compliance with industry best practices.
% 
However, none of these current programs and IAB standards address the accessibility of ads, such as readability by screen readers or keyboard navigation. 
% 
Including accessibility criteria in these guidelines would ensure that ads meet website accessibility standards. 
% 
Updating IAB standards to cover accessibility requirements would support assistive technologies and enhance compliance with website accessibility guidelines.
% 
When leasing an ad slot, the website developer is often provided with the option to enforce restrictions on the type of ads they want to display on their websites. Based on our findings, we advocate that this ad restriction should also include an option to host only WCAG-complaint ads. 

%%
\noindent\textbf{User-side accessibility tools.}
Recent advancements in large language models (LLMs) can significantly benefit accessibility tools by addressing common accessibility violations automatically. 
% 
For instance, when dealing with missing {\tt alt text} for images, LLMs can analyze the image's content and generate descriptive and contextually relevant {\tt alt text}. 
% 
These models can provide accurate descriptions by leveraging advanced image recognition and natural language processing capabilities, making the content more accessible to users with visual impairments. 
% Similar to screen readers, such methods are applicable on the user's side once the ad is served. 
However, hosting large-sized models in a browser extension is not feasible. Small, domain-specific language models are an active area of research, which can advance a browser's ability to auto-transform inaccessible ads into WCAG-complaint with minimal runtime cost.
%


% \noindent\textbf{Improving privacy with accessible ads.} Ads often raise privacy concerns due to misleading content and involuntary tracking from screen readers, as discussed in Section~\ref{sec:misrepesentation}. This particularly affects users with visual impairments and cognitive disabilities, who may be deceived by the ads' true intent. Existing ad blockers, like uBlock Origin, block all ads, affecting the revenue streams supporting free internet services. We advocate for research into methods that can help users separate privacy-violating ads from legitimate ones by tracking users' private data flow through the website's code to third-party URLs. Traditional static taint analysis and debugging can provide information to create accessible alt text, warning users with disabilities about malicious ads before they interact with them. 

%Ads are often associated with privacy concerns due to misleading ads and involuntary tracking due to screen readers' interaction with the websites, as demonstrated in Section~\ref{sec:misrepesentation}. This is especially concerning for users with visual impairment and cognitive disabilities who are deceived into interacting with ads as they struggle to interpret the ads’ true intent. Existing Ad blockers, such as uBlock Origin, block all ads from loading, which harms the revenue streams that support free internet services. We encourage research into methods that can distill privacy-violating ads from legitimate ads by tracking the dataflow of users' private information to third-party tracking URLs, as listed in the filter list. Traditional static taint analysis and debugging can offer information that can transformed into accessuble alt text to warn user with disability about the malaicvouis intent of the ads before they itneractn with them. 






%\todo{im not sure if llm in extension are even possible and there will be no-runtime cost}

% \noindent\textbf{Balancing accessibility and ad-delivery.}
% Blanket ad-blocking prevents all ad-serving technologies from delivering ads on websites, which might eliminate non-accessible ads. 
% % 
% However, while ad-blocking is a tool to manage excessive ads, it can undermine the goal of a free and open internet, which is essential for maintaining online content accessibility and sustainability. 
% % 
% Accessible ads are crucial for ensuring that users with disabilities can interact with content safely and effectively.
% % 
% By adhering to accessibility standards, ads not only foster a more inclusive web experience but also provide users with disabilities the necessary context and functionality for meaningful engagement with online advertisements. 
% % 
% Achieving a balance between ad support and accessibility is key to maintaining an equitable digital environment while sustaining the economic model of free Internet access.

%%


==> ICSE/parts/graveyard.tex <==
In this section, we describe the design and implementation details of our accessibility report collection pipeline. Our crawling infrastructure, based on a campus network in North America, comprised of a ??-node cluster with ?? cores at ??GHz, ??GB storage, and ??GB memory. Figure X provides an overview of the pipeline, which starts with automated website crawling using the Selenium web driver and using \textbf{IBM EEAC} chrome extension that generates accessibility reports for web pages. The features that the accessibility report gets, along with an example is shown in table ??. We first run this script on top 5k news websites, first without \textbf{uBlock Origin} chrome extension and then with the extension enabled. We get two accessibility reports for each website and then using those reports we compute the difference between the two on the basis of "Code" to identify violations that were introduced due to ads. We combine all the files containing the differences to form a single data frame on which further analysis is performed.

\subsection{Selenium Script}
The Selenium script automates accessibility testing of websites using the IBM EAAC extension in Chrome. It reads URLs from a text file and processes each to download and save the HTML content, both with and without the adblocker. The script configures a Chrome WebDriver with options to load the IBM accessibility extension and optionally the adblocker. It navigates to each website, interacts with the extension through DevTools, and saves the accessibility report, first with and then without the adblocker enabled, to a designated directory. We generate accessibility reports on landing pages of top 5k news websites using the IBM EAAC extension. We give a delay of 10 seconds on each web page to make sure the page is completely loaded and the browser window is opened in maximized mode. There is another 3 second delay to make sure DevTools is open and the extension is ready. Upon triggering the IBM EAAC extension, an additional delay of 20 seconds is introduced to ensure the complete execution of the extension. Finally, the reports are saved in a designated directory in xlsx format. If a URL causes an error, the process terminates, and the URL is marked as crashed.

\subsection{IBM EAAC Extension}
The IBM Easy Accessibility Extension (EAAC) enables users to generate accessibility reports for web pages. Once activated in a Chrome browser session, the extension conducts real-time analysis of webpage accessibility. It examines critical elements like color contrast, text size, and semantic structure to verify adherence to accessibility standards. When integrated with DevTools, the extension delivers precise insights into potential accessibility issues that require manual review, recommendations for enhancement and identification of accessibility violations. Users can interact with the extension to explore the accessibility report, which features actionable insights and highlighted areas requiring attention. The issues are categorized in following levels:
\begin{itemize}
    \item \textbf{Level 1 -} The most essential issues to address
    \item \textbf{Level 2 -} The next most important issues
    \item \textbf{Level 3 -} Necessary to meet requirements
    \item \textbf{Level 4 -} Further recommended improvements to accessibility
\end{itemize}
We used IBM EAAC Extension because not only it was including ads while generating the accessibility report but it could be easily integrated with chrome Devtools and provided a detailed accessibility report. 
\subsection{uBlock Origin Extension}
uBlock Origin is a widely acclaimed browser extension renowned for its robust ad-blocking capabilities. Developed as an open-source project, uBlock Origin operates by leveraging filter lists—lists of rules that dictate what elements (such as advertisements, trackers, and other undesirable content) should be blocked on web pages.  When a user visits a web page, uBlock Origin parses these filter lists and applies rules to decide which elements to block or allow based on their URLs and other criteria. This process occurs in real-time as the page loads, ensuring that unwanted content such as ads and tracking scripts are intercepted before they can display or execute.
\subsection{Dataset}
We generate accessibility reports for top 5k news websites. We only consider 2608 since these include both the versions of the accessibility report, with and without ad block. If either version is absent due to any reason, we skip that website. We get the difference between the two versions of the reports to get the issues that were exclusively present in the version without an ad blocker. There was a total of 164,306 issues of which 54,610 were violations, 32,345 were recommendations and 77,351 required review.

==> ICSE/parts/intro.tex <==
\section{Introduction}
\begin{figure*}[!t]
\centering
\begin{subfigure}{.295\textwidth}
    \fbox{\includegraphics[width=.95\linewidth]{images/normal.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (0.1,0.8) rectangle (5.2,1.8);
          \draw[red,thick,rounded corners] (0.6,0.4) rectangle (4.8,0.7);
    \end{tikzpicture}
    \vspace{-.2in}
    \caption{Control}
    \label{fig:normal}
\end{subfigure}
% \begin{subfigure}{.44\textwidth}
%     \includegraphics[width=.99\linewidth]{images/lighthouse.png}
%     % \vspace{-.04in}
%     \caption{Google's Lighthouse}
%     % \label{fig:lighthouse}
% \end{subfigure}
\begin{subfigure}{.34\textwidth}
    \fbox{\includegraphics[width=.95\linewidth]{images/adblock.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (4.7,0.5) rectangle (5.6,1);
    \end{tikzpicture}
    \vspace{-.18in}
    \caption{Accessibility without Ads}
    % \label{fig:noublock}
\end{subfigure}
\begin{subfigure}{.34\textwidth}
    \fbox{\includegraphics[width=.96\linewidth]{images/noadblock.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (4.6,0.5) rectangle (5.5,1);
    \end{tikzpicture}
    \vspace{-0.2in}
    \subcaption{Accessibility with Ads}
    % \label{fig:ublock}
    \end{subfigure}
% \vspace{-.09in}

\caption{Accessibility report for {\tt alaskasnewssource.com}, highlighting the count of accessibility violations, which are 126 when the website is visited without ads and 279 when inspected with ads.} 
\vspace{-3ex}
\label{fig:motivating-example}
\end{figure*} 


% \gulzar{We can look into combining the two paragraphs below.} 
Approximately 15\% of the global population has some form of disability, and their access to the internet depends largely on website accessibility. Many of these users rely on assistive technologies like screen readers, which require highly accessible websites (\eg properly labeled images) to function effectively\cite{brown1992assistive}.
The Web Content Accessibility Guidelines (WCAG) \cite{WCAG-21}, led by the World Wide Web Consortium (W3C), have driven efforts to improve website's accessibility. As a result, numerous tools and services now exist to test and enhance website accessibility \cite{kumar2021comparing,gleason2020twitter,zhang2021screen, prakash2024all}. While website's accessibility is gradually improving due to these tools, the accessibility of website advertisements (ads) remains largely unexamined. 

Website ads are the driving force behind the free and open Internet\cite{evans2009online}. Website developers integrate ads on their websites by leasing space to ad-serving technologies (\eg Taboola \cite{Taboola}) that serve user-relevant ads when a visitor accesses the site. Consequently, developers give up control over the ad content served on their websites and whether it meets WCAG accessibility guidelines.


\noindent {\bf Problem.} Including ads on a website poses several challenges in evaluating the website's accessibility. 
First, popular website accessibility tools, like Google Lighthouse \cite{Google-lighthouse}, do not include ads in their assessments, which overestimates accessibility in evaluation reports. 
Second, due to the dynamic nature of ad content, website developers cannot predict which ads will be served to users or whether those ads will adhere to WCAG guidelines. Even when a website developer makes the best effort to ensure WCAG compliance, ads can significantly deteriorate the overall accessibility of the website.
Third, inaccessible website ads prevent users with disabilities from accessing a significant portion of the website. This is especially alarming when ads pose privacy and security risks \cite{bashir2016tracing, englehardt2016online, eslami2018communicating,li2012knowing, rastogi2016these}, as they are more likely to lead to fraud, phishing, and scams.
Fourth, blanket ad blocking harms the free internet and causes fundamental equity issues by making ads completely unreachable. Accessible ads not only encourage a free and open internet but also equip users with disabilities with the necessary context for safe and informed interaction with ads.

\noindent {\bf Prior-work.} While website accessibility has been extensively studied\cite{hackett2003accessibility, campoverde2023accessibility, mohammadi2024accessibility, agrawal2019evaluating, teixeira2021diversity, fok2022large, milne2014accessibility, ross2018examining}, to date, no comprehensive study has examined the accessibility of website ads at a large scale, leaving a significant gap in our understanding of website accessibility as a whole.
%the accessibility of web ads has never been investigated in depth. 
Only three studies have examined digital ad accessibility, focusing on small datasets of platform-specific ads and solely on blind website users. He et al.\cite{he2024tend} studied only 500 ad screens within Android apps and introduced a tool for detecting accessibility violations. Similarly, prior work manually examined {\tt alt text} on 67 websites \cite{thompson2001accessibility} and used a survey to understand screen reader users' challenges with website ads \cite{10.1145/3597503.3639229}. With the prevalence of website ads and their potential safety risks, the impact of website ads on accessibility remains an open yet important question.


\noindent {\bf Contributions.} In this paper, we conduct the first-of-its-kind large-scale, in-depth investigation of website ad accessibility and its impact on overall website accessibility. We perform an automated analysis of 430K website elements with nearly 100K website ad elements on the top 5K news and media websites. We first seek to understand the prevalence of inaccessible ads on the website and how they impact the overall accessibility of websites.
We build an automated pipeline to rigorously analyze the accessibility of website elements and the ads using IBM Equal Access Accessibility Checker and state-of-the-art ad-blocker, uBlockOrigin. Among ads that adversely impact a website's accessibility, we analyze the accessibility violations in accordance with WCAG guidelines. Identifying such violations provides key insights into commonly overlooked accessibility guidelines in ads and determines whether these violations are prevalent only in ads. To inform developers about accessibility violations across different ad-serving technologies, we further analyze inaccessible ads with respect to the technologies serving them.

Ads are historically more likely to lead to fraud, phishing, and scams~\cite{li2012knowing, rastogi2016these}. Even when ads are accessible, we investigate whether the provided accessible information truly represents the content and intent of the ad. We utilize open-source CLIP (Contrastive Language–Image Pretraining) model \cite{OpenAI-Clip} to confirm whether the content of ad images aligns with the provided alternative text for accessible ads. For instance, users with visual impairments solely rely on alternate text to access website content; false and misrepresented alternatives can mislead such users into involuntary interaction with ads. The onus for addressing inaccessible and misleading ads falls on the website developer whose website is hosting such ads.

% \todo{mention about manual study}
% \noindent {\bf  Methodology.} We build extend IBM Equal Access IBM Equal Access Accessibility Checker to  We utilize a top-of-the-line ad blocker, uBlock Origin, to remove ads and measure website's accessibility both with and without ads. We extract the violations specific to ad elements by differencing website's accessibility both with and without ads.
% % pinpointing which accessibility violation are connected to specific ad elements on the website is difficult. We employ XYZ to automatically analyze accessibility reports and identify violations specifically linked to advertisements. 
% Second, we utilize a combination of existing databases \cite{easylist, easyprivacy} containing known ad-serving technologies for labeling ad elements. 
% % 
% 
% % 
% This also involves verifying whether the alternative text correctly defines the ad or not.
% % 
% Lastly, we manually inspect the consequences of interacting with these misleading ads to determine whether they collect user identifiers for invasive tracking.

\noindent {\bf Findings.}
Our analysis reveals that 75\% of websites have ads that frequently fail to comply with WCAG guidelines. On average, we observe  11 more accessibility violations due to ads. 
% 
We further categorize the most common WCAG guideline violations found in ads to illustrate their potential impact on individuals with disabilities. We identified 28 different WCAG guideline violations in ad elements, with 7 of these violations predominantly occurring in only ad elements. These violations are related to missing captions, missing focus order, and missing page language, all of which are critical in ensuring smooth navigation on a website. 
% 
Our analysis also identifies the ad-serving technologies responsible for the majority of these violations. We found that 52\% of websites use one of Google's ad-serving technologies (e.g., DoubleClick), which account for over 14K violations in their ad elements.
% 

We show that the misrepresentation of data in alternate texts compared to the actual image deceives users with visual impairments and cognitive disabilities, making it difficult for them to interpret the intent of the ads. We found that 27\% of ad images misrepresent their content and intent. Furthermore, our manual inspection of ads from top-50 news websites reveals that up to 94\% of the ads collect trackable user identifiers upon {\tt onmouseover}, {\tt onhover}, and {\tt onclick}  events. These events help assistive technologies identify website elements that a user with disability desires to access. Thus, navigating ads can compromise the privacy of assistive technology users. To the best of our knowledge, this is the first work that investigates the accessibility violations of website ads on a large scale. 
% 

\noindent {\bf Data Availability:} Our data is available at \url{https://zenodo.org/records/13137429}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\todo{Imp of Websites:} 
% About 15\% of the global population has some form of disability whose access to the internet depends on how accessible websites are. Many such users use assistive technologies like screen readers, which require highly accessible websites (e.g., properly labeled images) to function effectively~\cite{}. 
% %and include accessible digital content on websites is crucial 
% %Websites are essential in daily life, with millions available and billions of users relying on them ~\cite{?}. 
% % 
% %In practice, web developers often neglect accessibility when creating websites, leaving a significant portion of internet users in the dark.%: accessibility. 
% %% Therefore, it is essential for developers to ensure their websites are accessible to everyone, regardless of their abilities or preferred interaction methods.
% %% 
% %\todo{WCAG Guidelines:} 
% %Empirical studies show that accessibility issues are prevalent on real-world websites, leaving websites inaccessible for a significant portion of internet users. 
% %
% The Web Content Accessibility Guidelines (WCAG), led by the World Wide Web Consortium (W3C), have driven efforts to improve web accessibility.  As a result, numerous tooling and services test and improve the accessibility of websites today~\cite{}. 
% %
% While web accessibility is gradually improving due to these tools, the accessibility of {\em website advertisements} remains unexamined. 
% % 

% Web advertisements are the driving force behind free and open Internet, comprising nearly X\%  of the web content ~\cite{}. Web developers integrate ads on their webpage by leasing their website's space to ad technologies (e.g., Adsense~\cite{}) that serve user-relevant ads when a user visits a website.  Consequently, web developers give up control over what ad content will be served on their websites and if it will meet the WCAG accessibility guidelines. 

% Including ads on websites poses several accessibility challenges. First, popular web accessibility tools, like Google Lighthouse, do not include advertisements in their assessments, which overestimates accessibility scores. Second, the dynamic nature of ad content means website developers cannot predict which ads will be served to users, causing noticeable variation in accessibility scores. Therefore, even when a web developer makes the best effort to make the website WCAG complaint, ads can significantly deteriorate the overall accessibility score of the website. Third, inaccessible web advertisements cause additional problems for users with disabilities. As a result, users with disabilities are unable to access a significant portion of the website. This is especially alarming when ads pose privacy and security risks ~\cite{?}, as they are more likely to lead to fraud, phishing, and scams. Fourth, blanket blocked ads harm the free internet and cause fundamental equity issues by making ads completely unreachable. Accessible ads not only encourage free and open internet but also equip users with disabilities with the necessary context for safe and informed interaction with ads. 


% %  



% % %, security aspects ~\cite{?}, and user perceptions ~\cite{?}, but there is limited research on their impact on people with disabilities. 
% % % 

% % Evaluating the accessibility of advertisements on websites is challenging because 
% % % 
% % Another issue is that website developers often have limited control over the ads displayed, as they rely on ad-serving technologies like Taboola.
% % % 
% % This leaves manual checks as the primary method for assessing ad accessibility after deployment. 
% % % 
% % Additionally, the dynamic nature of ad content means website developers cannot predict which ads will be served to users, further complicating accessibility efforts.


 
% % State-of-the-art web accessibility tools, like Google Lighthouse, do not include advertisements in their assessments, resulting in incomplete accessibility scores. 









% %In the web ecosystem, websites have primarily two revenue-models: paid-subscriptions, advertisements, or a combination of both. 
% %  Advertisements have become an essential part of this ecosystem, forming a multi-billion-dollar market ~\cite{?}.




% %  Technology companies and organizations, led by initiatives from the World Wide Web Consortium (W3C), especially the Web Accessibility Initiative (WAI) and its Web Content Accessibility Guidelines (WCAG), are addressing these concerns to ensure web content is accessible.
% % 
% While web accessibility has been extensively studied~\cite{}, the accessibility of web ads has never been investigated in depth. Only three studies have investigated digital ad accessibility, however, on a very small dataset of platform-specific ads and for only blind web users. He et al.~\cite{?} studied only 500 ad screens within Android apps and introduced a tool for detecting accessibility issues. Similarly, prior work looked manually at only ALT tags of 67 websites ~\cite{}  and used a survey to understand screen reader users' challenges with web ads~\cite{}. With the prevalence of web advertisements and their potential safety risk, the impact of web ads on the accessibility of a website remains an open yet important question. 

% % Thompson and Wassmuth ~\cite{?} found that over half of the ads on 67 online newspaper websites lacked ALT tags.
% % Nengroo and Kuppusamy ~\cite{?} used questionnaires to assess but did not observe real-time interactions. 
% % 

% %%
% \todo{Our Work:} In this paper, we conduct the first large-scale, in-depth investigation on the accessibility of web ads and their impact on overall web accessibility. We perform an automated quantitative and qualitative analysis of nearly 100K web advertisement elements on the top 5000 news and media websites. We first seek to understand the prevalence of inaccessible ads on the web and how they impact the overall accessibility of websites.  
% Among those that adversely impact a website's accessibility score, we reason about the accessibility violations in accordance with the WCAG guidelines. Finding such violations provides key insight into commonly overlooked accessibility issues in ads and if and why they are prevalent only in ads. To inform developers about the accessibility issues with different ad-serving technologies, we further analyze the inaccessible ads with respect to the ad technologies serving them. Ads are historically more likely to lead to clickbait, fraud, phishing, and scams. Even when ads are accessible, we investigate if the provided accessible information truly represents the content and intent of the advertisements. For instance, users with visual impairments solely rely on such alternate descriptions to access web content; false and misrepresented alternates can mislead such users into involuntary interaction with ads. The onus of addressing inaccessible and misleading ads falls on the web developer whose website is hosting such ads.

% The first challenge is measuring precisely the accessibility of the ads, excluding the website's original elements. We utilize a top-of-the-line ad blocker called uBlockOrigin to remove advertisements and measure the webpage's accessibility both with and without ads. Another significant challenge involves pinpointing which accessibility issues are connected to which advertisement elements on the website. To address this, we employ XYZ to automatically analyze accessibility reports and identify violations specifically linked to advertisements. In order to determine the ad-serving technology, we utilize a combination of existing databases containing tracking URL lists and known hosting domains of ad technologies to trace the source of the ads. Finally, we utilize state-of-the-art open-source LLMs (Llama3) to confirm whether the content of ad images aligns with the provided alternative text for accessible ads. This also involves verifying whether the alternative text correctly identifies the ad as an advertisement. 



% %While previous studies on the accessibility of ads have been limited in scope and lack large-scale systematic research, our work addresses this gap with a comprehensive empirical


% %, both with and without advertisements, using an accessibility tool that accounts for ads.
% % 



==> ICSE/parts/methodology.tex <==

\section{Research Questions}
Given the proliferation of ads on popular websites, their impact on vulnerable users, and the gap in developers' understanding of ad accessibility, we aim to answer the following research questions:
% 
\begin{enumerate}
    \item \textbf{RQ1:} How do advertisements impact the accessibility guideline violations of websites?
    \item \textbf{RQ2:} What are the most common accessibility guideline violations found in advertisements?
    \item \textbf{RQ3:} Which ad-serving technologies frequently exhibit accessibility violations in their served advertisements?
    \item \textbf{RQ4:} How is information misrepresented in the alternate text of advertisements?
\end{enumerate}

\section{Methodology}
\label{sec:methodology}
To address the research questions, we designed an automated pipeline to inspect websites, identify accessibility violations in each element, extract violations specific to ad elements, and categorize them based on WCAG guidelines \cite{WCAG-21}.
% To address the research questions, we designed an automated pipeline to inspect websites, identify accessibility violations in each element, extract violations in ad-slot elements, and categorize them based on Web Content Accessibility Guidelines (WCAG)\cite{WCAG-21}. 
% 
Figure \ref{fig:overview} illustrates the overview of the process used in our empirical investigation, which is completely automated and packaged into a single measurement tool. 
% 
\begin{table}[t]
\small
    \centering
    \scalebox{0.8}{\input{tables/sample-report}}
    % \vspace{0.2in}
    \caption{Sample accessibility evaluation report detailing elements and associated violation information.}
    \label{table:report}
    \vspace{-0.25in}
\end{table}
\subsection{Websites Visited}
%% 
We visit the top 5K news and media category websites from SimilarWeb \cite{Similar-web}, using a custom Selenium (version 4.11.2) based automated website navigator running on Google Chrome (version 120.0.6099.129).  
% 
Prior literature has also focused on this category of websites because they have the most ads \cite{thompson2001accessibility,zeng2020bad,he2024tend}, offering the most breadth and coverage of ads. 
% 
For every website, we launch our automated website navigator to first visit the website and then eventually trigger the accessibility evaluation using the IBM accessibility tool, as explained in Section~\ref{sec:accessiblity-evaluation}. 
%
It takes approximately 30 seconds for a website to fully load (until the onLoad event is fired), on average, and an additional five minutes to ensure all ads are loaded before applying the accessibility checks.  
% 
We use a stateless crawling process, with all cookies and local browser states cleared between consecutive visits. 
% 
This approach helps ensure that the collected accessibility data accurately reflects the current state of the website without being biased by previous visits. 
% 
We visited all 5K websites in North America. 
% 

We crawl each website twice to obtain two accessibility evaluation reports for the same website:
\begin{enumerate}
    \item $Report (R_{with-ads})$: Accessibility report of the website with ads.
    \item $Report (R_{without-ads})$: Accessibility report of the website without ads.
\end{enumerate}
% 
$Report (R_{with-ads})$ contains the accessibility report for all elements on the website, including ad elements.
% 
$Report (R_{without-ads})$ contains the accessibility report for all elements on the website, excluding ad elements.
% 
Finally, we extract the $ Report (R_{only-ads})$ by differencing the 
$R_{with-ads}$ and $R_{without-ads}$, which represents the accessibility report for the ad elements only:
\begin{equation}
    \underbrace{R_{with-ads}}_{\text{Website elements with Ads}} - \underbrace{R_{without-ads}}_{\text{Website elements without Ads}} = \underbrace{R_{only-ads}}_{\text{Ad elements}}
\end{equation}
% 
\noindent\textbf{Why do we need this approach to find the accessibility of ads?} To date, there does not exist any tool that can identify and isolate accessibility scores for ad elements alone. 
% 
Ads can only be evaluated post-deployment because, during the development phase, ad-serving technology only requires reserved space on the website. 
% 
The actual ads only appear on the website based on user client profiling and real-time advertiser bidding. 
% 
We opt to evaluate these ads post-deployment on the client side to understand the true accessibility impact of ads, offering insights for developers and ad-serving technologies. 

\begin{table}[t]
\small
    \centering
    \scalebox{0.85}{\input{tables/dataset}}
    % \vspace{0.2in}
    \caption{Number of website elements with violations during the campaign, detailing ad elements by violation level and criteria.}
    \label{table:dataset}
    \vspace{-0.25in}
\end{table}
%%
\subsection{Blocking Website Advertisements}
To measure the website's accessibility without ads, we aim to load the website without any ads in our crawler, which requires removing all ads before performing accessibility evaluations. 
% 
We leverage a widely used, advanced ad-blocking tool called uBlock Origin\cite{uBlock-origin} to remove ads from a website before it completely loads in the browser. 
% 
uBlock Origin relies on a crowd-sourced filter list\cite{easylist, easyprivacy}, which are databases of rules and patterns that identify and block resources from commonly used ad-serving technologies. 
% 
Almost all ad blocking tools\cite{uBlock-origin, Adblockplus, adguard} rely on the same filter lists and, therefore, have more or less similar effectiveness in blocking ads.  
% 
Internally, when a user visits a website, the ad blocker scans the page and its resources, comparing URLs and scripts against its filter lists.
% 
If it detects elements associated with ad-serving technology, it prevents these elements from being loaded on the page. 
% 
This can involve blocking requests to known ad servers, hiding ad elements within the DOM, or preventing ad scripts from executing. 
%
As a result, the ad content is not displayed to the user, resulting in an ad-free website, which we use to perform accessibility evaluations, $R_{without-ads}$. 
%
Prior work\cite{castell2022demystifying} on the effectiveness of ad-blocking tools has shown that uBlock Origin is the most effective ad blocker. 

%%
\subsection{Accessibility Evaluation}
\label{sec:accessiblity-evaluation}
After the website loads, we automatically perform a rigorous accessibility evaluation using the IBM Equal Access Accessibility Checker \cite{IBM-accessibility}, a Chrome extension. 
% 
Initially, we use Google's Lighthouse\cite{Google-lighthouse}, commonly used for quality checks during development. 
% 
However, tools like Lighthouse, Axe \cite{Axe}, and Wave \cite{Wave} exclude ad elements by default, leading to inaccurate measurements for sites with ads. 
% 
Thus, we use the IBM checker to assess accessibility for all website elements, including ads.
% After the website loads completely, we automatically perform rigorous accessibility evaluation of the website using the IBM Equal Access Accessibility Checker \cite{IBM-accessibility}, offered as a Chrome browser extension.
% % 
% Initially, we leverage Google's built-in accessibility tool, Lighthouse\cite{Google-lighthouse}, which is widely used by web developers to perform quality checks on websites while it is being developed. 
% % 
% Unfortunately, Lighthouse and several existing like Axe \cite{Axe}, and Wave \cite{Wave}, by default, exclude ad elements during the accessibility measurements of the website. 
% % 
% Using such tools to measure $R_{with-ads}$ leads to incorrect measurements for the accessibility of websites with ads. 
% % 
% Therefore, we choose the IBM accessibility checker to compute accessibility evaluation report for all website elements, including ads.
%%
Internally, IBM's accessibility checker injects a content script into the website to interact with the website's DOM. 
% 
The content script scans the website's DOM to identify elements and runs a series of checks based on the following predefined rules such as WCAG 2.1 \cite{WCAG-21}.
% 
The results are intercepted by our automated website navigator and stored in separate storage for downstream analysis. 
% 

%%
\noindent\textbf{Accessibility Report.} 
Table \ref{table:report} shows a sample accessibility evaluation report with a detailed analysis of violations, including page title, URL, HTML element type, element code, XPath, WCAG checkpoint, and violation level. Each checkpoint corresponds to a specific WCAG criterion with a description of the violation.
% Table \ref{table:report} shows a sample accessibility evaluation report.
% % 
% It includes a detailed analysis of accessibility violations found on a website's elements, including the page title, URL, HTML element type, element code, XPath, WCAG checkpoint, and WCAG violation level.
% % 
% Each WCAG checkpoint corresponds to a specific criterion within the WCAG levels and includes a description of the violation.
% 
The WCAG level indicates the priority and severity of accessibility violations, categorized into three levels:
% 
\begin{itemize}
    \item \textbf{Level A:} These guidelines are fundamental for all websites. Non-compliance makes website content inaccessible to users with disabilities. For example, text alternatives for non-text content (WCAG 1.1.1) are crucial for users with visual impairments. Meeting Level A criteria is a top priority. 
    % most fundamental web accessibility features that all Websites must include. Non-conformance to Level A makes website content completely inaccessible to users with disabilities.  For example, providing text alternatives for non-text content (WCAG 1.1.1) is essential for users with visual impairments who rely on screen readers. Meeting Level A success criteria for a website is of the highest priority. 
    \item \textbf{Level AA:} These guidelines should be met by most websites. Conformance to Level AA significantly improves the accessibility of website content. For example, ensuring that text and images of text have a contrast ratio of at least 4.5:1 (WCAG 1.4.3) is crucial for users with visual impairments, including those with color blindness.
    % Conformance to Level AA significantly improves the accessibility of web content. For example, ensuring that text and images of text have a contrast ratio of at least 4.5:1 (WCAG 1.4.3) is crucial for users with visual impairments, including those with color blindness.
    \item \textbf{Level AAA:} These guidelines represent the highest website accessibility standards for full accessibility. For example, sign language interpretation for pre-recorded audio (WCAG 1.2.6) benefits deaf users. Level AAA conformance is not mandatory for WCAG compliance as it applies to specific content types. \textit{Note: These violations require manual assessment and are excluded from this analysis}.
    
    % For example, providing sign language interpretation for all pre-recorded audio content in synchronized media (WCAG 1.2.6) benefits users who are deaf and rely on sign language. Level AAA conformance is not required for a website to be WCAG compliant, as the included accessibility features are only applicable to specific types of content. \textit{Note that these violations cannot be evaluated automatically and require manual assessment, thus they are excluded from this analysis.}
\end{itemize}
%  

%$R_{with-ads}$ and $R_{without-ads}$ ,

\noindent\textbf{Extracting Ad-elements.} We first generate the two accessibility reports of each website in our dataset, $R_{with-ads}$ and $R_{without-ads}$.
% 
$R_{with-ads}$ represents the accessibility report of all the website elements, including ads, as illustrated in Figure \ref{fig:overview} \ding{202} - \ding{205}.
% 
$R_{without-ads}$ represents the accessibility report of all the website elements excluding ads, as illustrated in Figure \ref{fig:overview} \ding{202} - \ding{203}.
%
Finally, we automatically compare the two accessibility reports by first matching website elements based on their code and Xpath location, resulting in a list of website elements that are not ads (\ding{202} and \ding{203}). 
% 
We exclude these elements from $R_{with-ads}$, which results in an accessibility report of ads only, $R_{ads-only}$ as illustrated in Figure \ref{fig:overview} \ding{204} - \ding{205}.
% On average, it took two minutes to generate an accessibility report for a single instance of a website.
% 
We analyzed 430K unique HTML elements with accessibility violations across 5k websites, of which 23.1\% are ad elements.
% 
Computing accessibility reports is time-consuming and resource-intensive due to the extensive checks required on the rendered page, styling, and HTML structure.
% Computing accessibility reports is compute-intensive and time-consuming due to the wide range of checks that the accessibility checkers have to perform on both the rendered page and the underlying styling and HTML structure. 
% 
It also cannot be deployed on the cloud, as certain accessibility metrics can only be measured when active display is available for UI rendering.
% 
Therefore, analysis on the 5K website consumed more than 484 CPU hours to generate accessibility reports spanning 20.6 GB.  
% 
Table \ref{table:dataset} lists the number of website elements with violations that we interacted with during this campaign.
% 
Specifically, it details the ad elements with violations, categorizing them by the level and criteria of violations.
%


==> ICSE/parts/related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Accessibility of websites and mobile applications has been extensively studied \cite{hackett2003accessibility, campoverde2023accessibility, mohammadi2024accessibility, agrawal2019evaluating, teixeira2021diversity, fok2022large, milne2014accessibility, ross2018examining}. 
% 
Hackett et al. \cite{campoverde2023accessibility} used the Internet Archive’s Wayback Machine to demonstrate that websites have become progressively less accessible as their complexity has increased. 
% 
Teixeira et al. \cite{teixeira2021diversity} conducted a systematic literature review focusing on website accessibility within the tourism industry. 
% 
Similarly, Moreno et al. \cite{moreno2008guiding} proposed a method to improve website design for accessibility by addressing identified violations. 
% 
Fok et al. \cite{fok2022large} conducted a large-scale analysis of mobile applications to investigate how inaccessible user interfaces are. 
% 
Similarly, Milne et al. \cite{milne2014accessibility} and Ross et al. \cite{ross2018examining} found that missing or vague labels in mobile applications hinder screen readers from conveying information to visually impaired users.

%%
 Digital ads on websites and mobile applications are mainly studied for privacy-invasive targeted advertising mechanisms (\eg \cite{bashir2016tracing, englehardt2016online, eslami2018communicating}), malicious ads spreading malware or click fraud and phishing attacks (\eg \cite{li2012knowing, rastogi2016these}), and deceptive or manipulative content (\eg \cite{zeng2020bad}).
% 
However, there is very limited research specifically focused on the accessibility of online ads.
% 
He et al. \cite{he2024tend} conducted an empirical study on the accessibility of mobile ads for blind users in Android apps, identifying significant challenges such as missing {\tt alt text} for images, complex gestures problematic for screen readers, and ads that disrupt app functionality. 
% 
However, their analysis was limited to only 500 ad elements on mobile applications, so their insights are not applicable to website ads broadly.
% 
Similarly, Thompson et al. \cite{thompson2001accessibility} manually examined {\tt alt text} for ad elements on 67 news websites, while Chiou et al. \cite{10.1145/3597503.3639229} automatically detected reflow accessibility violations in website advertisements for keyboard users. Both studies are small-scale and on limited accessibility violations. 
% 
To date, the large-scale accessibility of website ads remains a significant and unresolved question.

%%
Several tools\cite{kumar2021comparing,gleason2020twitter,zhang2021screen, prakash2024all} have been developed to address accessibility issues. 
% 
Twitter A11y \cite{gleason2020twitter} is a browser extension designed to add alternative text to images on Twitter.
% 
Zhang et al. \cite{zhang2021screen} created a machine-learning model that infers accessibility metadata from mobile app screens, improving iOS VoiceOver functionality and enhancing accessibility for existing apps. 
% 
InstaFetch \cite{prakash2024all} is a browser extension that consolidates website content into a screen reader-friendly interface, allowing blind users to access information across multiple pages efficiently.
% 
while these tools may improve the accessibility of general website content, it is yet to be measured if these fully address the accessibility violation caused by the ads. 


%Studies done on mobile ads in Android Apps:

%[8] https://seal.ics.uci.edu/publications/2024_ICSE_AdMole.pdf

%[9] https://dl.acm.org/doi/pdf/10.1145/3491102.3502143

%[10] https://milnel2.github.io/files/mobileHealth.pdf

%[11] https://dl.acm.org/doi/pdf/10.1145/3234695.3236364

%[12] https://core.ac.uk/download/pdf/82110597.pdf

%These works focus on a range of accessibility concernss in Android apps, including labeling, touch target size, color contrast, and more:

%https://www.researchgate.net/publication/333625374_Accessibility_Assessment_in_Mobile_Applications_for_Android

%%https://ics.uci.edu/~iftekha/pdf/paper16.pdf

%https://www.researchgate.net/publication/333625374_Accessibility_Assessment_in_Mobile_Applications_for_Android

%https://ieeexplore.ieee.org/document/8918937

%https://www.researchgate.net/publication/317183694_Universal_Design_of_Mobile_Apps_Making_Weather_Information_Accessible

%https://dl.acm.org/doi/10.1145/3300176

%================================

% Works done on web accessibility



%[13] Literature review on University websites accessibility. 
%Link: https://link.springer.com/article/10.1007/s10209-021-00825-z

%[14] https://www.researchgate.net/profile/Gaurav-Agrawal-28/publication/332763704_Evaluating_Accessibility_and_usability_of_airline_websites/links/643e1aa02eca706c8b66a2ef/Evaluating-Accessibility-and-usability-of-airline-websites.pdf

%[15] This work analyzes prior studies done on educational websites accessibility. It analyzes 25 prior papers. 
%Link: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9092982

% [16] Power et al. found that only 50% of problems were addressed by the guidelines, revealing that meeting accessibility criteria does not ensure screen reader users have The Accessibility of Data Visualizations on the Web for Screen Reader Users access to the information. 
%Link: https://dl.acm.org/doi/10.1145/2207676.2207736

%Making memes accessibile
%Link: https://www.cs.cmu.edu/~jbigham/pubs/pdfs/2019/accessible-memes.pdf

%Accessibility in Visualization
%https://dl.acm.org/doi/abs/10.1145/3491102.3517630

%=================================

%Tools developed to improve accessibility

%Twitter: https://dl.acm.org/doi/abs/10.1145/3313831.3376728

%Mobile apps:
%https://dl.acm.org/doi/abs/10.1145/3411764.3445186



==> ICSE/parts/results.tex <==
\section{Results}
\label{sec:results}
\begin{figure}
    \centering
    \include{plots/rq1-violations-diff}
    \vspace{-0.4in}
    \caption{CDF plot of websites by accessibility guideline violations in ad elements (\roa).}
    \label{fig:cdf-scores}
    \vspace{-0.2in}
\end{figure}
%
\begin{figure}
    \centering
    \include{plots/rq1-violations-histogram}
    \vspace{-0.4in}
    \caption{Histogram of the number of websites by accessibility guideline violations in ad elements (\roa).}
    \label{fig:histogram-violations}
    \vspace{-0.2in}
\end{figure}
\subsection{RQ1: Impact of Advertisements on Accessibility Violations}
We first examine the impact of ads on the number of accessibility violations on websites.
% 
This analysis demonstrates how third-party ad content can lower a website's accessibility, which has several downstream consequences, such as potentially low search rankings on Google due to accessibility violations\cite{Seo-accessibility} in addition to the fundamental inclusivity issues for users with disabilities. 
% 
Figure \ref{fig:cdf-scores} presents the cumulative distribution of websites and their WCAG guideline violations of ad elements (\roa). 
%The accessibility violations in websites with ads consistently stay on the right of the accessibility violations in websites without ads. 
% This shows that websites containing ads almost always incur more WCAG guidelines violations. 
% 
Concretely, the average violation count is 106.2, with a median of 72, for websites without ads (\rwoa). 
% 
For websites with ads (\rwa), the average violation count increases to 118.1, with a median of 81.
% , indicating a 10.1\% increase in violations when advertisements are present.
% 
Overall, the average violation count for ad elements (\roa) is to 11.7. 
% 
While the magnitude of the increase in violations may not look drastic, it is important to understand that a single violation directly points to an accessibility issue of a website element that makes it inaccessible for at least one type of disabled website user. 
% 
As mentioned before, WCAG guidelines violations in ads are more challenging to address than the violations in original website content, as a developer can immediately act on violations from original website content, whereas, in the case of ads, it is infeasible for the developer to address the violation due to user-specific dynamic nature of ads. 
%

To further understand the number of violations caused by the ads on websites, we distribute websites with the number of violations caused by ads. 
% 
Figure \ref{fig:histogram-violations} displays the distribution of websites for one or more accessibility guideline violations.  
% 
We find that nearly 74.6\% of websites have at least one accessibility violation in their ad elements (\roa), and 66.7\% of websites have an increase in violations after including ads (\rwoa $\rightarrow$ \rwa).
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, nearly 75\% of websites show at least one accessibility violation attributed to ad elements, underscoring the need for further investigation into these violations.
 }
\end{tcolorbox}

%%
\begin{table}[t]
\small
    \centering
    \scalebox{0.97}{\input{tables/rq2-violations}}
    \caption{Top-10 Most prevalent violations in ad elements}
    \label{table:rq2-violations}
    \vspace{-0.25in}
\end{table}
\begin{figure}[!t]
\vspace{0.1in}
\begin{subfigure}{.28\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq2-normal.png}
    \caption{Focus Visible}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=.90\linewidth,height=2cm]{images/rq2-ad.png}
    \caption{Focus Not Visible}
\end{subfigure}

\caption{The blue highlighted border shows the focus on the San Diego news block in (a), but it is not visible on the ad element in (b).} 
% \vspace{-3ex}
\label{fig:rq2-focus}
\vspace{-0.2in}
\end{figure} 
% 
\subsection{RQ2: Common Accessibility Violations in Advertisements}
To further understand the reason behind the increase in violations caused by the ad elements on websites, we investigate the different types of violations, when these violations occur, and how common those are in ad elements.  
\lstdefinestyle{base}{
language=html,
moredelim=**[is][\color{red}]{@}{@},
moredelim=**[is][\color{darkgreen}]{~}{~},
numbers=left,
numberstyle=\tiny,
stepnumber=1,
numbersep=5pt,
escapechar=`
}
\begin{lstlisting}[caption={The corresponding {\tt <a>} tag for the aforementioned sponsored ad does not comply with WCAG on input criteria.},language=html, label={lst:on-input}, style=base]
<a id="aw0" target="_blank" href="https://googleads.g.doubleclick.net/pcs/click?....." onfocus="ss('aw0')" onmousedown="st('aw0')" onmouseover="ss('aw0')" onclick="ha('aw0')">
        <img src="https://tpc.googlesyndication.com/simgad/2522640214132067527" border="0" width="292" height="30" alt="" class="img_ad">  
</a>
\end{lstlisting}
%%
\subsubsection{Prevalent Violations in Ad Elements (\roa)}
%
This analysis provides insights into design-specific violations within ad elements and their potential implications.
% 
Table \ref{table:rq2-violations} highlights the most prevalent violations we found in ads across 5K websites.
%
Note that these ad elements with violations are rendered at runtime, preventing developers from addressing them during deployment.

%% 
\noindent\textbf{Focus Visible} is one of the most common violations. Focus visible results enforce that keyboard focus indicators are visible when styling elements like links or ad elements using CSS. 
% 
In other words, website elements currently focused on should be highlighted. 
% 
For example, on the website {\tt 10news.com}, we identified a Google Ads iframe that violates this rule, as depicted in Figure \ref{fig:rq2-focus}(b). 
% 
In \ref{fig:rq2-focus}(a), the website developer has correctly implemented the focus visible feature by highlighting website cards with a blue border and thus adheres to focus visible. 
% 
Under WCAG Success Criterion 2.4.7 (Focus Visible)\cite{WCAG-list}, focus indicators must always be visible, which benefits users with motor disabilities, visual impairments (including low vision), cognitive disabilities, and those relying on accessibility tools like screen readers.
% 
We observe that 54.1\% of the website ad elements have not implemented focus visible.
%


% \vspace{-0.2in}
\begin{figure}[t]
    \centering
      \fbox{\includegraphics[width=0.40\textwidth]{images/rq2-on-input.png}}
      \begin{tikzpicture}[overlay]
          \fill[black] (-2.4,2.4) rectangle (-0.4,3.);
          \draw[red,thick,rounded corners] (-7.5,0) rectangle (-0.18,1.3);
    \end{tikzpicture}
        \caption{The Fox News weather widget, featuring a sponsored ad element highlighted in a red box, does not comply with WCAG on input criteria.}
        \label{fig:rq2-on-input}
        \vspace{-0.3in}
\end{figure}
% 

\begin{figure*}[!t]
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-captions}
    \vspace{-.4in}
    \caption{Missing Captions}
    \label{fig:normal}
\end{subfigure}
\hspace{-.2in} % Adjust horizontal space
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-focus-order}
    \vspace{-.4in}
    \caption{Focus-order}
    % \label{fig:lighthouse}
\end{subfigure}
\hspace{-.2in} % Adjust horizontal space
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-language}
    \vspace{-.4in}
    \caption{Language of Page}
    % \label{fig:noublock}
\end{subfigure}
\caption{Violations are predominantly found in ad elements (\roa) rather than in website elements (\rwoa).} 
\vspace{-4ex}
\label{fig:rq2-cdf}
\end{figure*}
%%
\noindent\textbf{In Input} is the second most common violation in ad elements that fails to inform users when their input action will change the context i.e., navigating to a different page or opening a new window. 
% 
This requirement is mandated by WCAG Success Criterion 3.2.2 (On Input) \cite{WCAG-list}. 
% 
According to this criterion, user actions on an interface component should not automatically change the context without prior notification. Violating "on input" causes confusion or disorientation from unexpected context changes.
% According to this criterion, any user action on an interface component should not automatically change the context unless the user has been informed of this behavior beforehand.
% % 
% Violating "on input" can significantly impact users with cognitive disabilities, leading to confusion or disorientation when unexpected context changes occur without prior notification.
% 
We observe this violation on 47.1\% of the websites' ad elements.
% 
For example, on the website {\tt foxnews.com}, we identified an ad that violates this rule, as shown in Figure \ref{fig:rq2-on-input}.
% 
The red-highlighted ad has associated {\tt onclick}, {\tt onmouseover}, {\tt onmousedown}, and {\tt onfocus} events, as shown in Listing \ref{lst:on-input}.
% 
These events open a new window (target="\_blank"), but there is no indication in the link text or an accessible tag like {\tt aria-label} to inform users that a new window will be opened. 
% 
It is mandatory to inform users about changes in context to prevent disorientation.
% 

% \begin{figure}[h]
%     \centering
    
%     % Subfigure 1: Image with overlay
%     \begin{subfigure}[b]{0.40\textwidth}
%         \centering
%         \fbox{\includegraphics[width=\textwidth]{images/rq2-on-input.png}}
%         \begin{tikzpicture}[overlay]
%             \draw[red,thick,rounded corners] (-3.2,0.6) rectangle (3.5,1.4);
%         \end{tikzpicture}
%         \caption{on-input-example}
%         \label{fig:rq2-on-input}
%     \end{subfigure}
%     \hfill
%     % Subfigure 2: Code listing
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \lstdefinestyle{base}{
%             language=html,
%             moredelim=**[is][\color{red}]{@}{@},
%             moredelim=**[is][\color{darkgreen}]{~}{~},
%             numbers=left,
%             numberstyle=\tiny,
%             stepnumber=1,
%             numbersep=5pt,
%             escapechar=`
%         }
%         \begin{lstlisting}[caption={On Input Example}, language=html, label={lst:on-input}, style=base]
% <a id="aw0" target="_blank" href="https://googleads.g.doubleclick.net/pcs/click?....." onfocus="ss('aw0')" onmousedown="st('aw0')" onmouseover="ss('aw0')" onclick="ha('aw0')">
%         <img src="https://tpc.googlesyndication.com/simgad/2522640214132067527" border="0" width="292" height="30" alt="" class="img_ad">  
% </a>
%         \end{lstlisting}
%     \end{subfigure}
    
%     \caption{Combined figure with image and code listing}
%     \label{fig:combined}
% \end{figure}
% 

%%
% \noindent\textbf{In Context} is the third most common violation by ad elements where hyperlinks do not provide link text, labels, or images with text alternatives. 
% % 
% This requirement is mandated by the WCAG Success Criterion 2.4.4 (Link Purpose - In Context)\cite{WCAG-list}. 
% % 
% According to this criterion, the purpose of each link should be clear from the link text alone or from the link text in conjunction with its context. 
% % 
% This is crucial for users who depend on screen readers to understand the purpose of each link without having to click on it first.
% % 
% We observed this violation in 38.3\% of the websites' ad elements. 
% % 
% For example, on the website {\tt mediapost.com}, we identified an ad by  Smart AdServer that violates this rule, as shown in Figure \ref{fig:rq2-in-context}. 
% % 
% The sponsored ad is rendered using an {\tt <a>} and {\tt <img>} tag without {\tt alt-text}, as shown in Listing \ref{lst:in-context}. 
% % 
% This forces users with disabilities to click on the link without knowing the outcome beforehand, which is particularly problematic if the link redirects to scam or phishing websites.
% \vspace{-0.1in}
% % 
% \begin{figure}[h]
%     \centering
%       \fbox{\includegraphics[width=0.40\textwidth]{images/rq2-alt-tag.png}}
%         \caption{The Mediapost website features a sponsored ad element that does not comply with WCAG in-context criteria.}
%         \label{fig:rq2-in-context}
%         \vspace{-0.2in}
% \end{figure}
% % 
% % 
% \lstdefinestyle{base}{
% language=html,
% moredelim=**[is][\color{red}]{@}{@},
% moredelim=**[is][\color{darkgreen}]{~}{~},
% numbers=left,
% numberstyle=\tiny,
% stepnumber=1,
% numbersep=5pt,
% escapechar=`
% }
% \begin{lstlisting}[caption={The corresponding {\tt <a>} tag for the aforementioned sponsored ad does not comply with WCAG in-context criteria.},language=html, label={lst:in-context}, style=base]
% <a href="https://use1.smartadserver.com/click?..." target="_blank">
%     <img id="img_36497925" src="https://creatives.sascdn.com/diff/1909/advertiser/522511/WBNR96-CausalIQ-001-728x90dbl_0046e903-e3e2-4c44-afc9-a1f30c6f8fe0.gif" width="728" border="0" height="90">
% </a>
% \end{lstlisting}
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, we observed 28 different types of violations, with the most prevalent being Focus Visible (54\%), and In Input (47\%) across various websites. 
    % and In Context (38\%) across various websites.
 }
\end{tcolorbox}

% 


\subsubsection{Violations in Ad Elements (\roa) vs. Non-ads Website Elements \rwoa}
% 
This analysis highlights the accessibility violations that are specific to ad elements (\roa) but not quite prevalent in non-ad elements (\rwoa). 
% 
We compare violations from over 99K ad elements and 331K non-ad elements.
% 
Figure \ref{fig:rq2-cdf}(a-c) shows the distribution of websites with the three most commonly found violations in ad elements (\roa), which are not common in non-ads website elements (\rwoa).

%%
\noindent\textbf{Missing Captions} (WCAG 1.2.4 \cite{WCAG-list}) is one of the most common accessibility violations found more in ad elements  (\roa) than standard website elements  (\rwoa). 
% from plots: 100-83.6 and 100-91.7 
% 
This criterion requires that pre-recorded and live audio content in synchronized media (such as videos) includes captions.
% 
Captions are essential for users who are deaf, as they provide a text alternative to spoken dialogue and important audio information.
% 
On average, 16.4\% of ad elements (\roa) contain at least one instance of this violation, whereas only 8.3\% of website elements (\rwoa) exhibit the same violation. 
% 
In other words, ad elements (\roa) are 2$\times$ more likely to be missing captions than non-ads elements (\rwoa) on websites.

%%
\noindent\textbf{Focus Order} (WCAG 2.4.3 \cite{WCAG-list}) is found to be more prevalent in ad elements (\roa) than non-ads website elements (\rwoa).  
% from plots: 100-72.9 and 100-80.9
This criterion requires that the navigation order of interactive elements on a website is logical and intuitive, ensuring users can navigate through content in a predictable manner. 
% 
Proper focus order is crucial for users who rely on keyboard navigation, such as individuals with motor impairments or those using assistive technologies like screen readers. 
% 
Without a logical focus order, users may struggle to understand the structure of the page, miss important information, or find it difficult to interact with the content. 
%
On average, 27.1\% of ad elements (\roa) contain at least one instance of this violation, whereas only 19.1\% of website elements (\rwoa) exhibit the same violation.

%%
\noindent\textbf{Language of Page}  (WCAG 3.1.1 \cite{WCAG-list}) is another accessibility violation that is found more in ad elements than non-ad website elements. 
% 
This criterion requires that the primary language of a website element is clearly defined in the HTML. 
% 
Declaring the language is essential for users who rely on assistive technologies, such as screen readers, which use this information to provide accurate pronunciation and interpretation of the content. 
% 
Without the language of the page specified, users with visual impairments or cognitive disabilities may have difficulty understanding the content, leading to a less accessible and non-inclusive website experience. 
% from plots: 100-54.7 and 100-79.9 
On average, 45.3\% of ad elements (\roa) contain at least one instance of this violation, whereas only 2.1\% of website elements (\rwoa) exhibit the same violation.  
% 
Thus, ad elements (\roa) are 21$\times$ more likely to have this violation than non-ad elements (\rwoa).  
% 45.23/2.1
This significant difference points to the special ad accessibility case where website developers are not able to enforce language constraints on the ads served on their website due to the user-specific and dynamic nature of websites.  
% checkpoint.xlsx
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, we observed seven violations more common in ad elements (\roa) than in website elements (\rwoa): missing captions, incorrect focus order, undefined page language, insufficient text spacing, hover content violations, keyboard accessibility issues, and focus-related violations.
 }
\end{tcolorbox}


%%
\begin{table*}[t]
\small
    \centering
    \scalebox{0.9}{\input{tables/rq3-adv-violations}}
    % \vspace{0.2in}
    \caption{Top five ad-serving technologies with the highest number of violations.}
    \label{table:rq3-adv-violations}
    \vspace{-0.25in}
\end{table*}
%
\subsection{RQ3: Most Prevalent Ad-Serving Technologies on Websites with Ad Serving Violations}
We investigate the ad-serving technologies that deliver ads on websites with the most accessibility violations. 
% 
This analysis aims to guide website developers in selecting ad-serving technologies that comply with WCAG guidelines. 
% 
Additionally, it encourages ad-serving technologies to prioritize accessibility considerations before delivering ads on websites.
% 
Table \ref{table:rq3-adv-violations} lists the top ad-serving technologies prevalent on websites with the highest number of violations in ad elements (\roa). 

%%
\noindent\textbf{Taboola}  is a content discovery platform that promotes personalized content recommendations across websites. 
% 
In our investigation, it is found on 8.2\% of the inspected websites with a total of 18K violations.
% 
Common ad violation is related to guideline 1.1.1 \cite{WCAG-list}, which mandates that all content must have a text alternative for non-text content, found in 5,699 ads.
% 
Another common violation is related to guideline 3.2.2 \cite{WCAG-list}, which mandates providing adequate feedback when an action opens a new window or changes the context.
% 
This guideline is violated in 5,057 ads. 
% 
Lastly, guideline 2.4.7 \cite{WCAG-list}, which requires visible focus indicators for interface components to assist users navigating with keyboards or alternative devices, is violated in 4,658 ads served by Taboola.

%%
\noindent\textbf{DoubleClick} 
%The first two most prevalent ad-serving technologies are owned by Google.
% 
is Google's ad management platform, optimizing digital ad campaigns. 
% 
In our investigation, it is found on 31.5\% of inspected websites with a total of 10K violations.
% 
Common ad violations include not informing users when their input action will open a new window or change context (Guideline 3.2.2) \cite{WCAG-list}, which is found in 3,369 ads.
% 
Another common DoubleClick violation is related to guideline 2.4.4 \cite{WCAG-list}, which ensures links have clear, context-independent purposes,  benefiting screen reader users. 
% 
This guideline is violated in 3,344 ads.
% 
Lastly, Guideline 2.4.7 \cite{WCAG-list} mandates visible focus indicators for interface components, aiding users navigating with keyboards or alternative devices, and is violated in 1,675 ads served by DoubleClick.

%%
\noindent\textbf{RevContent} is an ad-serving technology that delivers personalized ad recommendations across various websites. 
% 
In our investigation, it is found on 6.5\% of inspected websites with a total of 3K violations.
% 
Common ad violations include not informing users when their input action will open a new window or change context (Guideline 3.2.2) \cite{WCAG-list}, which is found in 1,375 ads.
% 
Another common violation is related to guideline 2.4.1 \cite{WCAG-list}, which ensures that all functionality is accessible from a keyboard.
% 
This guideline is violated in 1,113 ads.
% 
Additionally, guideline 1.2.1 \cite{WCAG-list}, which requires that all multimedia content has a synchronized captioning or a transcript, is violated in 232 ads served by RevContent.

% \noindent\textbf{Google Syndication} is found on 20.4\% of websites.
% % 
% Common ad violations include failing to meet Guideline 2.4.7, which mandates visible focus indicators for interface components, found in 1,844 ads.
% % 
% Guideline 1.1.1 mandates that all non-text content (e.g., images) have text alternatives that convey their purpose. 410 ads served by syndication violate this guideline.
% % 
% Guideline 4.1.2 ensures that interactive elements are programmatically determinable for users relying on assistive technologies, and it is violated in 25 ads.

%%
% \noindent\textbf{OpenX}  is an advertising technology company that operates a real-time bidding platform for digital advertising. 9.4\% of websites contain ads served by OpenX.
% % 
% Common ad violations include failing to meet Guideline 2.4.1, which ensures direct access to primary content for sequential navigation, found in 668 ads.
% % 
% Guideline 2.4.7 mandates visible focus indicators, which was violated in 118 ads.
% % 

% \gulzar{Can we add taboola as well since it has the most violations?}
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, 52\% of websites using Google's ad-serving technologies violate WCAG guidelines across over 14K ad elements. Taboola serves the most ad elements with accessibility violations.
 }
\end{tcolorbox}

%%
\subsection{Misrepresentation of Alt Text in Advertisements}
\label{sec:misrepesentation}
Among the ads that do not lead to accessibility violation, we investigate the accessible information associated with ads that truly represents the intext and content of the ad. 
% 
Prior work privacy implications of ads~\cite{book2013longitudinal, book2015empirical, Alrizah19IMCerrorsMisunderstandings,Le21anticvndss,Bashir:2018:TCC:3278532.3278573} and malvertising~\cite{sood2011malvertising, xing2015understanding, arrate2020malvertising} show that clickbait~\cite{li2024attention,ahmad2024review} and false ads~\cite{handler1929false} can lead to scams, phishing, and fraud.  
% 
Analyzing alternate texts of otherwise accessible ads is important because it highlights how effective alternate texts are in effectively conveying the content of ads to users with disabilities.

%%
We start by extracting {\tt <img>} tags with alt text from the ads' HTML and collecting their {\tt src} values, which contain the image URLs. Next, we use the CLIP (Contrastive Language–Image Pretraining) model~\cite{OpenAI-Clip} to assess the relevance between images and their alt text. CLIP encodes images and text into a shared embedding space, allowing us to compute the cosine similarity between them. We classify alt text as redundant if the cosine similarity is below 0.5, which is the optimal threshold reported in previous research \cite{ahmad2024scs}. This approach efficiently evaluates the semantic alignment between visual and textual data.
% We start by extracting {\tt <img>} tags with alt text from the ads's HTML and collecting their {\tt src} values, which contain the URLs of the loaded images. 
% % We then compare these URLs against EasyList, a widely used database of tracking urls maintained by most ad blockers. 
% % If a URL appears in EasyList, it is identified as an advertisement.
% % 
% Next, we use the CLIP (Contrastive Language–Image Pretraining) model~\cite{OpenAI-Clip} to assess the relevance between images and their textual descriptions. 
% % 
% CLIP encodes both images and text into a shared embedding space, allowing us to compute the cosine similarity between these embeddings.
% % 
% We determine the relevance of the alt text to the image based on this similarity score. 
% % 
% Specifically, if the cosine similarity is below 0.5, we classify the alt text as redundant with respect to the image. 
% % 
% The cosine similarity threshold of 0.5 is previously reported to be the optimal threshold \cite{ahmad2024scs}. 
% % 
% This approach provides a robust and efficient means to evaluate the semantic alignment between visual and textual data.

%%
Overall, across 5K websites,  we find 9,827 ad images with alt text.
% 2665/9827
Of these, 27.1\% of ads have a cosine similarity score below 0.5, indicating a low level of similarity between the text and the ad image.
% 
For example, Figure \ref{fig:rq5-misrepresentation}(a) shows an image of shoes on a bench, served by Taboola on {\tt wsfa.com}, but the alt text describes foxes stealing footwear. This alt text mimics a news headline to confuse users, with a cosine similarity score of 0.33.
% 
Similarly, Figure \ref{fig:rq5-misrepresentation}(b) shows a hotel image on {\tt clickorlando.com}, but the alt text describes hotels turned into apartments for affordable housing. This alt text also resembles a news headline,  with a cosine similarity score of 0.28.
% For example, Figure \ref{fig:rq5-misrepresentation}(a) shows an image of several pairs of shoes placed on a bench, which is an ad served by Taboola Ad-serving technology on {\tt wsfa.com}. 
% % 
% However, its alt text describes a story about "foxes accused of stealing crocs and sandals from campers, after many pairs were found at a den". 
% % 
% The alt text is intentionally designed to mimic a news headline in order to confuse users visiting news websites.
% % 
% The image and the alt text have a cosine similarity score of 0.33, indicating a significant mismatch.
% % 
% Similarly, Figure \ref{fig:rq5-misrepresentation}(b) shows an image of a hotel, but the alt text describes distressed hotels turned into apartments for affordable housing on {\tt clickorlando.com}.
% % 
% Again, the alt text mimics a news headline in order to confuse users visiting news websites.
% % 
% The image and the alt text have a cosine similarity score of 0.28, indicating a significant mismatch.
% 
The alt texts of these ads do not disclose that they are ads and not the content served by the website. 
% They are often presented as news stories to deceive users, making them appear as legitimate content. 
% This can be especially problematic on news websites, where users expect genuine news stories, not advertisements masquerading as such. 
% 
Users may only realize it is an ad after performing actions like pressing enter to open the link, only to be redirected to a page outside the original domain. 
% 
Malicious and false ads represented as news in alt text can redirect to scam and phishing websites, compromising the safety of users with disabilities who struggle to assess a website's trustworthiness. 
%
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, 27\% of the nearly 10K ads have alt text that misrepresents ad image's content and intent.
 }
\end{tcolorbox}
% 
\begin{figure}[!t]
\vspace{0.1in}
\begin{subfigure}{.23\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq5-taboola.png}
    \caption{Alt-text: Foxes accused of stealing Crocs, sandals from campers after many pairs found at den.}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq5-cloudnary.png}
    \caption{Alt-text: Distressed hotels turned into apartments for affordable housing.}
\end{subfigure}

\caption{Misrepresentation of alt-text in image tags of ads.} 
\vspace{-0.3in}
\label{fig:rq5-misrepresentation}
\end{figure} 

%%
%% Privacy implication of having inaccessible ads
\noindent\textbf{Privacy implication of misleading advertisements.} We manually inspect the consequences of interacting with these misleading ads to determine if any user identifiers are collected for invasive tracking {\tt onhover}, {\tt onmouseover}, or when the user presses enter (for tabbable access) on these ads. 
% 
These three events are key resources for assistive technologies like screen readers to collect accessible information from website elements and deliver it to users using them  


% 
Prior research has shown that network traffic resulting from interacting with ads may contain user identifiers in headers \cite{rieder2024beyond, bujlow2015web}, cookies \cite{munir2023cookiegraph, amjad2024blocking}, and parameters \cite{munir2023purl}. 
% 
These identifiers can be used to trace a user's browsing activity on the web, violating their privacy. 
%Although these identifiers are encrypted, popular 
Lists maintained by ad-blockers identify specific headers\cite{Headers}, cookies\cite{CookieList}, and parameters\cite{AdguardBlockParam} as tracking identifiers for users. 
% 
We compare our network traffic from manually interacting with ads on the top 50 news websites against these lists to identify any tracking of user identifiers. 
% 
Our results show that on 94\% of websites, at least one tracking identifier is sent to an external server by hovering, and on 98\% of websites, at least one tracking identifier is sent to an external server by pressing enter on the ads. 
% 
Both events are essential actions that screen readers perform to read and announce website elements' content. None of the actions are necessary to access ads for regular users. 
%On hover, we do not find any trackable user identifiers transmitted through cookies and headers, but 84 different query parameters are sent to external servers. 
%In contrast, when pressing enter, 340 cookies, 12 headers, and 865 different query parameters are identified as trackable user identifiers using the lists.
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} On 94\% of websites, hovering sends tracking data to external servers, forcing users with disabilities to compromise privacy to navigate ad content, unlike regular users.
 }
\end{tcolorbox}

==> ICSE/parts/validitiy.tex <==
% \vspace{-0.15in}
\section{Threat to validity}
\label{sec:validity}
% 
\noindent\textbf{Internal validity.}
Our analysis in Section~\ref{sec:results} involves collecting ad elements (\roa) by differencing website elements without ads (\rwoa) from those with ads (\rwa). 
% 
However, various confounding factors may influence \roa.
% 
For instance, some websites dynamically fetch different elements, including ads, on each visit.
% 
Consequently, website elements loaded in \rwa might not appear in \rwoa. 
% 
Other factors include changes in behavior due to the environment (\eg browser and host OS), visit time, and location.
% 
To minimize this threat, we perform the two visits in quick succession and maintain consistent environments across different states, ensuring the same location, browser, and stateless crawls.

%%
\noindent\textbf{External validity.} 
% 
The IBM Equal Access Accessibility Checker \cite{IBM-accessibility} on different browsers might produce different accessibility violations due to the browser's built-in features, such as Safari's default blocking of certain ad-serving technologies \cite{Safari-ITP}. 
% 
We conduct our experiments using the Chrome browser with a Chrome-based extension, which is the most widely used browser, to minimize this threat.

%%
\noindent\textbf{Construct validity.}
We collect the website's elements at page load time and do not capture changes in accessibility violations triggered by user interactions such as scrolling and clicking. This is a general limitation of dynamic analysis that is challenging to overcome due to the numerous navigation and interaction scenarios on websites. 

==> ICSE/tables/clauses.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{3.5cm}|>{\raggedright\arraybackslash}p{10cm}|}
\hline
\textbf{Clause} & \textbf{Text} \\
\hline
1.1.1 & Non-text Content \\
1.1.1 & Non-text Content; 4.1.2 Name, Role, Value \\
1.2.1 & Audio-only and Video-only (Prerecorded); 1.2.2 Captions (Prerecorded); 1.2.4 Captions (Live) \\
1.3.1 & Info and Relationships \\
1.3.1 & Info and Relationships; 4.1.2 Name, Role, Value \\
1.3.1 & Info and Relationships; 3.3.2 Labels or Instructions \\
1.3.2 & Meaningful Sequence \\
1.3.3 & Sensory Characteristics \\
1.3.5 & Identify Input Purpose \\
1.4.1 & Use of Color \\
1.4.3 & Contrast (Minimum) \\
1.4.4 & Resize text \\
1.4.12 & Text Spacing \\
1.4.13 & Content on Hover or Focus \\
2.1.1 & Keyboard \\
2.1.1 & Keyboard; 2.4.3 Focus Order \\
2.1.2 & No Keyboard Trap \\
2.2.1 & Timing Adjustable \\
2.4.1 & Bypass Blocks \\
2.4.2 & Page Titled \\
2.4.4 & Link Purpose (In Context); 4.1.2 Name, Role, Value \\
2.4.6 & Headings and Labels \\
2.4.7 & Focus Visible \\
2.4.7 & Focus Visible; 3.2.1 On Focus \\
2.5.3 & Label in Name \\
3.1.1 & Language of Page \\
3.2.1 & On Focus \\
3.2.2 & On Input \\
3.3.2 & Labels or Instructions \\
4.1.2 & Name, Role, Value \\
\hline
\end{tabular}


==> ICSE/tables/dataset.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{1.2cm}|>{\raggedright\arraybackslash}p{1cm}|>{\raggedright\arraybackslash}p{4.9cm}|>{\raggedleft\arraybackslash}p{1cm}|}
     \cline{1-4}
     {\bf Violation } & {\bf Element} & {\bf WCAG} & {\bf Count}\\ 
     \cline{1-4}
        \multirow{2}{*}{Overall} & All & - & 430,497 \\
                  & Ad & - & 99,422 \\
        \cline{1-4}
        \multirow{3}{*}{Levels} & \multirow{3}{*}{Ad} & A  & 80,220 \\
                &  & AA  & 43,591 \\
                
        \hline
        \multirow{30}{*}{Criterion} & \multirow{30}{*}{Ad} & 2.4.7 Focus Visible& 41,110 \\ &  & 2.4.1 Bypass Blocks& 37,357 \\ 

                &  & 3.2.2 On Input & 26,629 \\
                & & 1.1.1 Non-text Content& 16,387 \\
                &  & 4.1.2 Name, Role, Value& 15,712 \\
                &  & 2.4.4 Link Purpose (In Context)& 7,714 \\
                &  & 1.3.4 Orientation& 6,493 \\
                &  & 1.3.1 Info and Relationships& 6,118 \\
                &  & 2.1.1 Keyboard& 6,026 \\
                &  & 2.4.3 Focus Order& 3,575 \\
                &  & 1.4.3 Contrast (Minimum)& 2,890 \\
                &  & 2.5.3 Label in Name& 1,190 \\
                &  & 1.2.1 Audio-only and Video-only& 1,147 \\
                &  & 1.2.4 Captions (Live)& 1,144 \\
                &  & 1.4.1 Use of Color& 1,021 \\
                &  & 3.3.2 Labels or Instructions& 269 \\
                &  & 1.3.3 Sensory Characteristics& 92 \\
                &  & 3.1.1 Language of Page& 60 \\
                &  & 1.4.12 Text Spacing & 26 \\
                &  & 1.4.4 Resize text& 21 \\
                &  & 2.1.2 No Keyboard Trap& 17 \\
                &  & 3.2.1 On Focus& 13 \\
                &  & 2.4.2 Page Titled& 6 \\
                &  & 2.4.6 Headings and Labels& 6 \\


                
                &  & 1.3.2 Meaningful Sequence& 3 \\
                
                
                &  & 1.3.5 Identify Input Purpose& 2 \\
                &  & 2.2.1 Timing Adjustable & 2\\
                &  & 1.4.13 Content on Hover& 1 \\
                

                
     \cline{1-4}
\end{tabular}

==> ICSE/tables/methodology-example_report.tex <==
\begin{tabular}{|p{1.5cm}|p{6.8cm}|}
\hline
\textbf{Feature} & \textbf{Example} \\
\hline
Page title & Atlanta news, Georgia news, Breaking news from The Atlanta Journal-Constitution - AJC.com \\
\hline
Page URL & \url{https://www.ajc.com/} \\
\hline
Scan Label & scan\_1 \\
\hline
Issue ID & 2748300732 \\
\hline
Issue Type & Violation \\
\hline
Toolkit level & 1 \\
\hline
Checkpoint & 1.1.1 Non-text Content \\
\hline
WCAG level & A \\
\hline
Rule & img\_alt\_valid \\
\hline
Issue & The image has neither an accessible name nor is marked as decorative or redundant \\
\hline
Element & img \\
\hline
Code & \texttt{<img style="display: block; padding: 0px; margin: 0px; border-width: 0px; min-width: 0px; min-height: 0px; max-width: none; max-height: none; -webkit-tap-highlight-color: rgba(0, 0, 0, 0); user-select: none; box-sizing: content-box; height: 100\%; width: 100\%; top: 0px; left: 0px; position: absolute;" src="https://clipcentric-a.akamaihd.net/file/1846203/master/1720505441/RhmEzmzh?f=auto" draggable="false">} \\
\hline
\end{tabular}


==> ICSE/tables/rq2-violations.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{6.8cm}|>{\raggedright\arraybackslash}p{1.2cm}|}
\hline
\textbf{Violation in Ad elements (\roa) } & \textbf{Websites} \\
\hline
Check the keyboard focus indicator is visible when using CSS declaration for 'border' or 'outline' & 2,708 \\
\hline
Inform the user when their input action will open a new window or otherwise change their context & 2,358 \\
\hline
 Hyperlink has no link text, label or image with a text alternative & 1,915 \\
\hline
 Verify \texttt{<frame>} content is accessible & 1,808 \\
\hline
Confirm the element should be tabbable and if so, it becomes visible when it has keyboard focus & 1,632 \\
\hline
Content is not within a landmark element & 1,605 \\
\hline
Verify there is a way to bypass blocks of content that are repeated on multiple Web pages & 1,490 \\
\hline
Confirm Windows high contrast mode is supported when using CSS to include, position or alter non-decorative content & 1,427 \\
\hline
Page detected as HTML, but does not have a 'lang' attribute & 1,374 \\
\hline
Inline frame does not have a 'title' attribute & 1,310 \\
\hline
\end{tabular}



==> ICSE/tables/rq3-adv-violations.tex <==
\begin{tabularx}{\textwidth}{|p{1.8cm}|p{1.4cm}|l|l|l|X|l|}
    \hline
    \textbf{Domain} & \textbf{Company} & \textbf{Websites}& \textbf{Violations} & \textbf{WCAG } & \textbf{Description} & \textbf{Count} \\
    \hline
    \multirow{3}{*}{taboola.com} & \multirow{3}{*}{Taboola} & \multirow{3}{*}{411}& \multirow{3}{*}{17,522} & 1.1.1  & All non-text content have text alternatives to ensure accessibility for users who rely on assistive technologies. & 5,699 \\
    \cline{5-7}
    &&&& 3.2.2  & User inputs should not trigger unexpected changes or disruptions in content. &  5,057 \\
    \cline{5-7}
    &&&& 2.4.7& Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 4,658\\
    \hline
    \multirow{3}{*}{doubleclick.net} & \multirow{3}{*}{Google} & \multirow{3}{*}{1,577} & \multirow{3}{*}{10,108}& 3.2.2  & User inputs should not trigger unexpected changes or disruptions in content. & 3,369 \\
    \cline{5-7}
    &&&& 2.4.4  & The purpose of a link is clear from its context, ensuring users understand where the link will take them. & 3,344 \\
    \cline{5-7}
    &&&& 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 1,675\\
    \hline
    
    %%
    \multirow{3}{*}{revcontent.com} & \multirow{3}{*}{RevContent} & \multirow{3}{*}{325}& \multirow{3}{*}{3,204} & 3.2.2 & User inputs should not trigger unexpected changes or disruptions in content. & 1,375 \\
    \cline{5-7}
    &&&& 2.4.1  & Users can bypass repetitive content, such as navigation menus, to access the main content more efficiently. & 1,113\\
    \cline{5-7}
    &&&& 1.2.1  & Text alternatives/captions for prerecorded audio and video content. & 232\\
    \hline
    %%
    \multirow{3}{*}{\parbox{1.5cm}{googlesyndica\\tion.com}} & \multirow{3}{*}{Google} & \multirow{3}{*}{1,021}& \multirow{3}{*}{2,339} & 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 1,844 \\
    \cline{5-7}
    &&&& 1.1.1 & All non-text content have text alternatives to ensure accessibility for users who rely on assistive technologies. &  410 \\
    \cline{5-7}
    &&&& 4.1.2  &  User interface elements have proper names, roles, and values to ensure they are accessible and understandable by assistive technologies. & 25\\
    \cline{5-7}
    \hline
    %%
    \multirow{3}{*}{google.com} & \multirow{3}{*}{Google} & \multirow{3}{*}{365}& \multirow{3}{*}{2,209} & 3.2.2 & User inputs should not trigger unexpected changes or disruptions in content. & 569 \\
    \cline{5-7}
    &&&& 4.1.2 &  User interface elements have proper names, roles, and values to ensure they are accessible and understandable by assistive technologies. &  516 \\
    \cline{5-7}
    &&&& 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 504\\
    \cline{5-7}
    \hline
\end{tabularx}

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/abstract.tex <==
\begin{abstract}
Website accessibility is essential for inclusiveness and regulatory compliance. Although third-party advertisements (ads) are a vital revenue source for free web services, they introduce significant accessibility challenges. Leasing a website's space to ad-serving technologies like DoubleClick results in developers losing control over ad content accessibility. Even on highly accessible websites, third-party ads can undermine adherence to Web Content Accessibility Guidelines (WCAG).
%, especially for visually impaired users who cannot distinguish original content from ads, increasing the risk of exploitation such as phishing and scams. Therefore, developers must address the accessibility impact of ads during web development.
We conduct the first-of-its-kind large-scale investigation of 430K website elements, including nearly 100K ad elements, to understand the accessibility of ads on websites. 
% 
We seek to understand the prevalence of inaccessible ads and their overall impact on the accessibility of websites.
% 
Our findings show that 67\% of websites experience increased accessibility violations due to ads, with common violations including Focus Visible (WCAG 2.4.7), and On Input (WCAG 3.2.2). 
% 
Popular ad-serving technologies like Taboola, DoubleClick, and RevContent often serve ads that fail to comply with WCAG standards. 
% 
Even when ads are WCAG compliant, 27\% of them have alternative text in ad images that misrepresents information, potentially deceiving users. 
% 
Manual inspection of a sample of these misleading ads revealed that user-identifiable data is collected on 94\% of websites through interactions, such as hovering or pressing enter.
% Further assessment of the privacy risk of ads reveals that interacting with ads through hovering and pressing enter resulted in the collection of user-identifiable data on 94\% of the websites. 
% 
Since users with disabilities often rely on tools like screen readers that require hover events to access website content, they have no choice but to compromise their privacy in order to navigate website ads. 
% 
Based on our findings, we further dissect the root cause of these violations and provide design guidelines to both website developers and ad-serving technologies to achieve WCAG-compliant ad integration.

% Our manual inspection of 50 websites revealed that






% Our findings show that 67\% of websites experience a notable increase in accessibility violations due to advertisements.
% The most common types of violations in advertisements include Focus Visible (WCAG 2.4.7), On Input (WCAG 3.2.2), and In Context (WCAG 2.4.4). 
% Additionally, we demonstrate that many popular ad-serving technologies, such as DoubleClick, Taboola, and Facebook, often fail to comply with WCAG standards for websites.
% Even when an ad is WCAG-compliant, we find that 27\% of the alt text in ad images misrepresents information, potentially deceiving users. 
% 
% 

% 



% Web accessibility is crucial for maintaining inclusiveness and meeting regulatory requirements.  
% % 
% While third-party advertisements (ads) are a key source of revenue for free web services, they pose significant accessibility challenges. 
% % 
% By leasing digital space on websites to ad-serving technologies like DoubleClick, developers forfeit control over the accessibility of ad content. 
% % 
% Inaccessible third-party ads may compromise website accessibility.  visually impaired users' ability to differentiate original content from ads. 
% %This increases the risk of exploitation, including phishing and scams. 
% % 
% Therefore, web developers must ensure that standards for websites, specifically the WCAG guidelines, during web development.


%Web accessibility is crucial for digital inclusivity and regulatory compliance. Third-party advertisements, while key for revenue in free web services, pose accessibility challenges. When developers use ad-serving technologies like DoubleClick, they lose control over ad content accessibility. This can undermine even ADA-compliant webpages, especially for visually impaired users relying on screen readers to navigate content. The inability to distinguish ads from original content increases vulnerability to phishing and scams. Developers must therefore consider and address the impact of ads on accessibility during web development.

% Free and open internet relies on third-party advertisements on websites to generate revenue. 
% % 
% By leasing digital space to ad-serving technologies like DoubleClick, developers lose control over the accessibility of ad content.
% % 
% Even if a webpage is ADA-compliant, third-party ads can undermine its accessibility, particularly for visually impaired users who cannot distinguish original content from ads when using assistive technologies like screen readers. 
% % 
% This increases the risk of exploitation, including phishing and scams. %In the US, over 84 million people have disabilities, yet a significant space on web pages is still not accessible to users without impairments. 
% % 
% Making web applications accessible is crucial for maintaining inclusiveness and is often a regulatory requirement. Therefore, during web development, developers must understand and address the accessibility impact of serving ads on their web pages.
% %

% We conduct the first large-scale, in-depth investigation to understand the accessibility of web advertisements from a web developer's perspective. 
% % 
% Our findings show that website advertisements increase accessibility violations by X\%.
% % 
% The most common types of violations in advertisements include X, Y, and Z. 
% % 
% We also demonstrate that many popular ad-serving technologies often fail to comply with ADA standards. 
% % 
% Even when an Ad is ADA-compliant, we find that 27\% of the alt-text in ad images misrepresents information, deceiving users.
% % 
% Assistive technologies like screen readers utilize {\tt onhover} events to let users access web content. We manually inspected 50 websites by interacting with misleading ads through hovering and clicking and found that X\% collected user-identifiable data. Thus, users with disabilities have no choice but to compromise their privacy in order to navigate the web.
% % 
% The findings of this work highlight the limitations of existing tools in measuring the true accessibility of the webpage and the precautions that web developers need to take when incorporating ads in webpages. 


%of leasing digital space to ad-serving technologies that comply with accessibility standards and encourage these technologies to improve the accessibility of their ads.

% Gulzar's abstract
% The free and open internet thrives by hosting third-party content, such as ads, that enable developers to earn revenue. To host an advertisement, web developers lease digital space on their web pages to ad agencies, such as Google and Taboola, who then serve advertisements on that space when a user visits the webpage. Inadvertently, web developers give up control of the web page's component serving ads and, therefore, are unable to verify the accessibility of significant content on their webpage. Even when the originally developed webpage claims to be ADA-compliant and accessible, the third-party inaccessible ads can severely harm the accessibility of the web page when served to the user. This is especially problematic because visually impaired users cannot distinguish organic content from advertisements, which is more likely to lead to exploitation, including phishing, fraud, and scams. In the US alone, over 84 million individuals live with some form of disability, yet modern webpages primarily cater to users without impairments.

% We conducted the first large-scale, in-depth investigation of 5,000 websites to understand the accessibility of web advertisements through the lens of a web developer. Using state-of-the-art, code-level content-blocking techniques, we measured the impact of advertisements on website accessibility and how exactly they deteriorate the browsing experience for visually impaired users. By combining investigations on ad accessibility issues with tracing web advertisements to their ad-serving agency, we identified the ad-serving technologies that most frequently deteriorate the accessibility of webpages. Users with disabilities rely on assistive technologies like screen readers to navigate web pages. A critical issue is the lack of proper labeling for third-party content. If an advertisement is accessible via alternate text, we used a large language model to verify if the alternate description of the ad truly conveys its intent as well as the content of the ad image. Our investigation reveals that web advertisements increase accessibility violations by 12\%, where more than half of the X number of ads are completely invisible to users with visual impairments. Among the ads with alternate descriptions, nearly 27\% of those have misrepresented alternate text, misleading users into interacting with ads that may violate their privacy.

% The free and open internet thrives by hosting third-party content, such as ads, that enable developers to earn revenue. To host an advertisement, web developers lease digital space on their web pages to ad agencies, such as Google and Taboola, who then serve advertisements on that space when a user visits the webpage. Inadvertently, web developers give up control of the web page's component serving ads and, therefore, are unable to verify the accessibility of significant content on their webpage. Even when the originally developed webpage claims to be ADA-compliant and accessible, the third-party inaccessible ads can severely harm the accessibility of the web page when served to the user. This is especially problematic because visually impaired users cannot distinguish organic content from advertisements, which is more likely to lead to exploitation, including phishing, fraud, and scams.  In the US alone, over 84 million individuals live with some form of disability, yet modern webpages primarily cater to users without impairments. 

% We performed the first large-scale, in-depth investigation of 5,000 websites to understand the accessibility of web advertisement through the lens of a web developer. Using state-of-the-art, code-level content-blocking techniques, we measured the impact of advertisements on website accessibility and how exactly they deteriorate the browsing experience for visually impaired users.   By combining investigations on ad accessibility issues with tracing web advertisements to its ad-serving agency, we identify the ad-serving technologies that most frequently deteriorate the accessibility of webpages. Users with disabilities rely on assistive technologies like screen readers to navigate web pages. A critical issue is the lack of proper labeling for third-party content.  If an advertisement is accessible via alternate text, we use the large language model to verify if the alternate description of the ad truly converts its intent as well as the content of the ad image.  Our investigation reveals that web advertisements increase accessibility violations by 12\%, where more than half of the X number of ads are completely invisible to users with visual impairments. Among the ads with alternate descriptions, nearly 27\% of those have misrepresented alternate text, misleading users into interacting with ads that may violate their privacy.


\end{abstract}


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/background.tex <==
\begin{figure}[!t]
% \vspace{0.1in}
\begin{subfigure}{.23\textwidth}
    \fbox{\includegraphics[width=.99\linewidth, height=2.6cm]{images/ad-issues-sample.png}}
    \caption{Accessibility Violations in Ad Slots of Taboola.}
\end{subfigure}
\hspace{.05in}
\begin{subfigure}{.23\textwidth}
    \fbox{\includegraphics[width=.99\linewidth]{images/ad-screenreader.png}}
    \caption{Ads are not accessible to users relying on screen readers.}
\end{subfigure}
\caption{Violation identified in Taboola ad slots and its impact on how screen reader users experience the website.} 
\vspace{-4ex}
\label{fig:ad-issues-sample}
\end{figure} 
\begin{figure*}[h]
    \centering
      \includegraphics[width=0.9\textwidth]{images/overview.png}
      %  \put(-392,5){{\ding{202}}}
      %  \put(-316,5){{\ding{203}}}
      % \put(-250,5){{\ding{204}}}
      % \put(-193,5){{\ding{205}}}
      % \put(-126,5){{\ding{206}}}
      % \put(-9,5){{\ding{207}}}
        \caption{Overview of our methodology involving generating accessibility reports for each website with (\rwa) and without ads (\rwoa), then comparing them to isolate and analyze the accessibility violations caused by only ads ($R_{ads-only}$).}
        \label{fig:overview}
        \vspace{-.2in}
\end{figure*}
\section{Motivating Example}
\label{sec:motivation}
% 
This section presents a case study showing how some ads on websites violate accessibility guidelines and affect the overall website's accessibility.
%can deteriorate the accessibility of the website. 
Alaska's News Source, {\tt alaskasnewssource.com}\cite{alaskanews}, provides local news, weather updates, sports coverage, and community events for the state of Alaska.
%
It is ranked 14\textsuperscript{th} in the top 5K in the news and media category.
% 
In the stock Chrome browser, this website shows numerous ads in ad slots—three at the top and one at the bottom, as seen in Figure \ref{fig:motivating-example}(a). 
% 
The top slots are served by Taboola\cite{Taboola} and the bottom by Google Ads\cite{Google-ads}.
% When loaded in the stock chrome browser, this website contains numerous advertisements placed in ad slots---three ads in the top slot and one ad on the bottom slot---as seen in Figure \ref{fig:motivating-example}(a). 
% % 
% These ad slots are filled by two different ad-serving technologies. Taboola\cite{Taboola} serves the top-one slots, and Google Ads\cite{Google-ads} serves those on the bottom.


\noindent\textbf{Website accessibility without ads.} 
In the first step, we generate the accessibility report for {\tt alaskasnewssource.com} by computing the violation count without including any ads.
% 
We remove ads from the website to emulate the website development stage, where website developers are unaware of the precise ads that will be served by the ad-serving technologies. 
% 
This is a common practice employed by many website quality and accessibility checkers like Google Lighthouse \cite{Google-lighthouse} that do not include ads in their accessibility evaluations. 
% 
We use IBM's accessibility checker chrome extension, a tool used by over 20K developers\cite{IBM-accessibility}, mainly because it evaluates all website elements, including ad elements. 
% 
To remove ads from the website, we deploy the uBlock Origin's Chrome extension, which has over 700K users\cite{uBlock-origin}, to block all ads on the website.  
%
As seen in Figure \ref{fig:motivating-example}(b), all ads on {\tt alaskasnewssource.com} are removed, and the accessibility checker reports 126 violations.
% 
For example, the element in Listing \ref{lst:motivation} violates the WCAG 2.4.4 (Link Purpose) \cite{WCAG-list} guideline because it lacks descriptive link text, label, or an image with a text alternative. 
% 
The guideline requires that links must have a clear purpose that users can understand, especially when the link is not accompanied by any other textual context. 
% 
This can be resolved by adding {\tt aria-label="Download the Alaska's News Source Streaming Apps"} to this tag by developer. 
% 
\lstdefinestyle{base}{
language=html,
moredelim=**[is][\color{red}]{@}{@},
moredelim=**[is][\color{darkgreen}]{~}{~},
numbers=left,
numberstyle=\tiny,
stepnumber=1,
numbersep=5pt,
escapechar=`
}
\begin{lstlisting}[caption={Anchor tag missing descriptive text},language=html, label={lst:motivation}, style=base]
<a data-tb-link="" target="\_self" rel="" href="https://www.alaskasnewssource.com/page/how-to-download-the-alaskas-news-source-streaming-apps/" class="link | text-reset d-block h-100 w-100">
\end{lstlisting}
% 
Most accessibility violations can easily be addressed by the developer with simple refactoring of the website's code (\ie HTML, CSS, and JS). 

\noindent\textbf{Website accessibility with ads.} Next, we compute accessibility report for {\tt alaskasnewssource.com} by computing the violation count with ads, as displayed to the user.
% 
This setting allows us to demonstrate the increase in the violations attributed to ads on the website.

% 
Figure \ref{fig:motivating-example}(c) shows that ads appear on the website as they did on a normal visit. 
% ((Second Value – First Value) ÷ First Value) x 100%
The accessibility checker reports 279 violations, showing a 121.4\% change in the violation count. 
% 
Given that the only difference between the two websites is the presence of ads, it is reasonable to attribute the increase in accessibility violations to the ads.
% 
We further examine specific violations related to ads, particularly concerning the ad slots Taboola serves. 
% 

Figure \ref{fig:ad-issues-sample}(a) shows violations identified by the accessibility checker across three ad slots for Taboola (highlighted with a red circle around their title and short description).
% 
This violates the WCAG 2.1.1 (Keyboard) guideline\cite{WCAG-list} because the element cannot be interacted with using a keyboard alone.
% 
All ad images are designed with a {\tt link role}, which does not include a tabbable element. 
% 
Thus, users who rely on keyboard navigation cannot directly access these elements. 
% 
Additionally, most of these ad images do not include alternate text to make them accessible for visually impaired users.   
% 
We further test the accessibility of these ads with  Google's Chrome Vox screen reader\cite{Chrome-vox}.
% 
Vox only announces {\tt image for Taboola advertising unit} on tab focus without reading the title and short description of each ad. 
% 
Figure \ref{fig:ad-issues-sample}(b) shows how the website and ads appear to visually impaired users using screen readers, leaving ads' content mostly inaccessible except the two vague alternate texts.
%


\textbf{\textit{It is difficult for a website developer to anticipate and address ad accessibility violations as these violations are non-deterministic and occur after the deployment of the website. }} 
% 
In the case of {\tt alaskasnewssource.com}, ads are negatively impacting accessibility, which raises the concern of whether such an effect is prevalent across all ads: (1) if yes, then what kinds of violations do they cause? and (2) if not, then does the accessible information in these ads adequately represent their content? Similarly, it is useful to know which ad-serving technologies are serving more inaccessible ads.


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/citations.tex <==
\begin{thebibliography}{00}

\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.









\end{thebibliography}

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}
\label{sec:conclusion}

Website ads are an integral part of a website and are essential for supporting free Internet; however, they often fail to meet basic accessibility standards.
This paper presents the first extensive study on the accessibility issues of website ads. Our research reveals that 67\% of websites show a noticeable increase in accessibility violations due to ads. We also discovered that popular ad-serving technologies do not adhere to the WCAG guidelines when displaying ads, and nearly one-quarter of ads that do comply with WCAG guidelines have misleading alt text.
Our findings provide insight into the challenges faced by website developers in integrating ads while maintaining accessibility. This research suggests ways for developers to enforce accessibility standards to lessen the impact of ads on overall website's accessibility.

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/discussion.tex <==
\section{Discussion and Takeaways}
\label{sec:discussion}
% 
Based on our empirical investigation, we provides insights for website developers and ad-serving technologies to address ad accessibility violations and highlights future research avenues for improving the website experience for users with disabilities.
% Based on our empirical investigation, we draw insights and takeaways for web developers and ad-serving technologies to help address accessibility issues in web ads.
% We also discover avenues for future research on developer tools to make the internet more inclusive and accessible and improve the web experience for users with disabilities. 

%%
\noindent\textbf{Accessibility-promoting ad integration for website developers.}
Ad integration is crucial for ad-driven websites. Developers must ensure high accessibility and WCAG compliance, which can be a regulatory requirement\cite{WCAG-21}. Once published, the developer cannot modify the website to address ad-related accessibility issues since new ads may introduce different violations. Developers can ensure two key aspects to improve ad accessibility during integration.
% Ad integration is a critical step in the development of ad-driven websites. When the website serves ads, it is the responsibility of the website developer to ensure high accessibility and WCAG compliance, which, in certain cases, is a regulatory requirement\cite{WCAG-21}. Once an ad slot is placed on the website and the website is published, the developer cannot modify or refractor the website's code to improve ad-related accessibility issues since each visit to the website brings a new ad, which may encounter a different accessibility violation. Website developers can ensure two key things to improve ad accessibility during ad integration.
% 
First, they can inject JavaScript to enforce CSS rules (using {\tt !important}) to implement basic checks on WCAG Type A violations. 
% 
For instance, a script can be added to ensure all text elements have sufficient color contrast. Such a script can be triggered on {\tt onload} events to detect certain accessibility violations and address them appropriately, if possible.  
% 
Some Type AA violations can also be addressed by injecting similar checks in the JavaScript, such as ensuring all interactive elements are keyboard accessible.
% 
Secondly, developers can run accessibility checks on their websites post-deployment (similar to our analysis) to analyze ad elements and derive specific self-correcting strategies to address those concerns.


%and address any remaining accessibility issues.
% \gulzar{1. Why ads are inaccessible? is it advertiser or publisher or web developer? 2.  automated accessibility enhancing  tools exist, but they only work on the developer side and at the client side; the violation will be different for every load. Anticipating accessibly for ads is hard. }
%%
\noindent\textbf{Accessibility strategies for ad-serving technologies.}
Website developers integrate ads on their websites by leasing ad space to ad-serving technologies. 
% 
These ad-serving technologies often enroll in programs such as the Acceptable Ads program \cite{Acceptable-ads} and adhere to guidelines set by the Interactive Advertising Bureau (IAB) \cite{IAB}.
% 
The Acceptable Ads Program promotes non-intrusive ad formats that respect user experience, requiring adherence to specific display guidelines. 
% 
The IAB sets comprehensive standards for digital advertising, including ad formats, measurement, and data privacy, ensuring compliance with industry best practices.
% 
However, none of these current programs and IAB standards address the accessibility of ads, such as readability by screen readers or keyboard navigation. 
% 
Including accessibility criteria in these guidelines would ensure that ads meet website accessibility standards. 
% 
Updating IAB standards to cover accessibility requirements would support assistive technologies and enhance compliance with website accessibility guidelines.
% 
When leasing an ad slot, the website developer is often provided with the option to enforce restrictions on the type of ads they want to display on their websites. Based on our findings, we advocate that this ad restriction should also include an option to host only WCAG-complaint ads. 

%%
\noindent\textbf{User-side accessibility tools.}
Recent advancements in large language models (LLMs) can significantly benefit accessibility tools by addressing common accessibility violations automatically. 
% 
For instance, when dealing with missing {\tt alt text} for images, LLMs can analyze the image's content and generate descriptive and contextually relevant {\tt alt text}. 
% 
These models can provide accurate descriptions by leveraging advanced image recognition and natural language processing capabilities, making the content more accessible to users with visual impairments. 
% Similar to screen readers, such methods are applicable on the user's side once the ad is served. 
However, hosting large-sized models in a browser extension is not feasible. Small, domain-specific language models are an active area of research, which can advance a browser's ability to auto-transform inaccessible ads into WCAG-complaint with minimal runtime cost.
%


% \noindent\textbf{Improving privacy with accessible ads.} Ads often raise privacy concerns due to misleading content and involuntary tracking from screen readers, as discussed in Section~\ref{sec:misrepesentation}. This particularly affects users with visual impairments and cognitive disabilities, who may be deceived by the ads' true intent. Existing ad blockers, like uBlock Origin, block all ads, affecting the revenue streams supporting free internet services. We advocate for research into methods that can help users separate privacy-violating ads from legitimate ones by tracking users' private data flow through the website's code to third-party URLs. Traditional static taint analysis and debugging can provide information to create accessible alt text, warning users with disabilities about malicious ads before they interact with them. 

%Ads are often associated with privacy concerns due to misleading ads and involuntary tracking due to screen readers' interaction with the websites, as demonstrated in Section~\ref{sec:misrepesentation}. This is especially concerning for users with visual impairment and cognitive disabilities who are deceived into interacting with ads as they struggle to interpret the ads’ true intent. Existing Ad blockers, such as uBlock Origin, block all ads from loading, which harms the revenue streams that support free internet services. We encourage research into methods that can distill privacy-violating ads from legitimate ads by tracking the dataflow of users' private information to third-party tracking URLs, as listed in the filter list. Traditional static taint analysis and debugging can offer information that can transformed into accessuble alt text to warn user with disability about the malaicvouis intent of the ads before they itneractn with them. 






%\todo{im not sure if llm in extension are even possible and there will be no-runtime cost}

% \noindent\textbf{Balancing accessibility and ad-delivery.}
% Blanket ad-blocking prevents all ad-serving technologies from delivering ads on websites, which might eliminate non-accessible ads. 
% % 
% However, while ad-blocking is a tool to manage excessive ads, it can undermine the goal of a free and open internet, which is essential for maintaining online content accessibility and sustainability. 
% % 
% Accessible ads are crucial for ensuring that users with disabilities can interact with content safely and effectively.
% % 
% By adhering to accessibility standards, ads not only foster a more inclusive web experience but also provide users with disabilities the necessary context and functionality for meaningful engagement with online advertisements. 
% % 
% Achieving a balance between ad support and accessibility is key to maintaining an equitable digital environment while sustaining the economic model of free Internet access.

%%


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/graveyard.tex <==
In this section, we describe the design and implementation details of our accessibility report collection pipeline. Our crawling infrastructure, based on a campus network in North America, comprised of a ??-node cluster with ?? cores at ??GHz, ??GB storage, and ??GB memory. Figure X provides an overview of the pipeline, which starts with automated website crawling using the Selenium web driver and using \textbf{IBM EEAC} chrome extension that generates accessibility reports for web pages. The features that the accessibility report gets, along with an example is shown in table ??. We first run this script on top 5k news websites, first without \textbf{uBlock Origin} chrome extension and then with the extension enabled. We get two accessibility reports for each website and then using those reports we compute the difference between the two on the basis of "Code" to identify violations that were introduced due to ads. We combine all the files containing the differences to form a single data frame on which further analysis is performed.

\subsection{Selenium Script}
The Selenium script automates accessibility testing of websites using the IBM EAAC extension in Chrome. It reads URLs from a text file and processes each to download and save the HTML content, both with and without the adblocker. The script configures a Chrome WebDriver with options to load the IBM accessibility extension and optionally the adblocker. It navigates to each website, interacts with the extension through DevTools, and saves the accessibility report, first with and then without the adblocker enabled, to a designated directory. We generate accessibility reports on landing pages of top 5k news websites using the IBM EAAC extension. We give a delay of 10 seconds on each web page to make sure the page is completely loaded and the browser window is opened in maximized mode. There is another 3 second delay to make sure DevTools is open and the extension is ready. Upon triggering the IBM EAAC extension, an additional delay of 20 seconds is introduced to ensure the complete execution of the extension. Finally, the reports are saved in a designated directory in xlsx format. If a URL causes an error, the process terminates, and the URL is marked as crashed.

\subsection{IBM EAAC Extension}
The IBM Easy Accessibility Extension (EAAC) enables users to generate accessibility reports for web pages. Once activated in a Chrome browser session, the extension conducts real-time analysis of webpage accessibility. It examines critical elements like color contrast, text size, and semantic structure to verify adherence to accessibility standards. When integrated with DevTools, the extension delivers precise insights into potential accessibility issues that require manual review, recommendations for enhancement and identification of accessibility violations. Users can interact with the extension to explore the accessibility report, which features actionable insights and highlighted areas requiring attention. The issues are categorized in following levels:
\begin{itemize}
    \item \textbf{Level 1 -} The most essential issues to address
    \item \textbf{Level 2 -} The next most important issues
    \item \textbf{Level 3 -} Necessary to meet requirements
    \item \textbf{Level 4 -} Further recommended improvements to accessibility
\end{itemize}
We used IBM EAAC Extension because not only it was including ads while generating the accessibility report but it could be easily integrated with chrome Devtools and provided a detailed accessibility report. 
\subsection{uBlock Origin Extension}
uBlock Origin is a widely acclaimed browser extension renowned for its robust ad-blocking capabilities. Developed as an open-source project, uBlock Origin operates by leveraging filter lists—lists of rules that dictate what elements (such as advertisements, trackers, and other undesirable content) should be blocked on web pages.  When a user visits a web page, uBlock Origin parses these filter lists and applies rules to decide which elements to block or allow based on their URLs and other criteria. This process occurs in real-time as the page loads, ensuring that unwanted content such as ads and tracking scripts are intercepted before they can display or execute.
\subsection{Dataset}
We generate accessibility reports for top 5k news websites. We only consider 2608 since these include both the versions of the accessibility report, with and without ad block. If either version is absent due to any reason, we skip that website. We get the difference between the two versions of the reports to get the issues that were exclusively present in the version without an ad blocker. There was a total of 164,306 issues of which 54,610 were violations, 32,345 were recommendations and 77,351 required review.

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/intro.tex <==
\section{Introduction}
\begin{figure*}[!t]
\centering
\begin{subfigure}{.295\textwidth}
    \fbox{\includegraphics[width=.95\linewidth]{images/normal.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (0.1,0.8) rectangle (5.2,1.8);
          \draw[red,thick,rounded corners] (0.6,0.4) rectangle (4.8,0.7);
    \end{tikzpicture}
    \vspace{-.2in}
    \caption{Control}
    \label{fig:normal}
\end{subfigure}
% \begin{subfigure}{.44\textwidth}
%     \includegraphics[width=.99\linewidth]{images/lighthouse.png}
%     % \vspace{-.04in}
%     \caption{Google's Lighthouse}
%     % \label{fig:lighthouse}
% \end{subfigure}
\begin{subfigure}{.34\textwidth}
    \fbox{\includegraphics[width=.95\linewidth]{images/adblock.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (4.7,0.5) rectangle (5.6,1);
    \end{tikzpicture}
    \vspace{-.18in}
    \caption{Accessibility without Ads}
    % \label{fig:noublock}
\end{subfigure}
\begin{subfigure}{.34\textwidth}
    \fbox{\includegraphics[width=.96\linewidth]{images/noadblock.png}}
    \begin{tikzpicture}[overlay]
          \draw[red,thick,rounded corners] (4.6,0.5) rectangle (5.5,1);
    \end{tikzpicture}
    \vspace{-0.2in}
    \subcaption{Accessibility with Ads}
    % \label{fig:ublock}
    \end{subfigure}
% \vspace{-.09in}

\caption{Accessibility report for {\tt alaskasnewssource.com}, highlighting the count of accessibility violations, which are 126 when the website is visited without ads and 279 when inspected with ads.} 
\vspace{-3ex}
\label{fig:motivating-example}
\end{figure*} 


% \gulzar{We can look into combining the two paragraphs below.} 
Approximately 15\% of the global population has some form of disability, and their access to the internet depends largely on website accessibility. Many of these users rely on assistive technologies like screen readers, which require highly accessible websites (\eg properly labeled images) to function effectively\cite{brown1992assistive}.
The Web Content Accessibility Guidelines (WCAG) \cite{WCAG-21}, led by the World Wide Web Consortium (W3C), have driven efforts to improve website's accessibility. As a result, numerous tools and services now exist to test and enhance website accessibility \cite{kumar2021comparing,gleason2020twitter,zhang2021screen, prakash2024all}. While website's accessibility is gradually improving due to these tools, the accessibility of website advertisements (ads) remains largely unexamined. 

Website ads are the driving force behind the free and open Internet\cite{evans2009online}. Website developers integrate ads on their websites by leasing space to ad-serving technologies (\eg Taboola \cite{Taboola}) that serve user-relevant ads when a visitor accesses the site. Consequently, developers give up control over the ad content served on their websites and whether it meets WCAG accessibility guidelines.


\noindent {\bf Problem.} Including ads on a website poses several challenges in evaluating the website's accessibility. 
First, popular website accessibility tools, like Google Lighthouse \cite{Google-lighthouse}, do not include ads in their assessments, which overestimates accessibility in evaluation reports. 
Second, due to the dynamic nature of ad content, website developers cannot predict which ads will be served to users or whether those ads will adhere to WCAG guidelines. Even when a website developer makes the best effort to ensure WCAG compliance, ads can significantly deteriorate the overall accessibility of the website.
Third, inaccessible website ads prevent users with disabilities from accessing a significant portion of the website. This is especially alarming when ads pose privacy and security risks \cite{bashir2016tracing, englehardt2016online, eslami2018communicating,li2012knowing, rastogi2016these}, as they are more likely to lead to fraud, phishing, and scams.
Fourth, blanket ad blocking harms the free internet and causes fundamental equity issues by making ads completely unreachable. Accessible ads not only encourage a free and open internet but also equip users with disabilities with the necessary context for safe and informed interaction with ads.

\noindent {\bf Prior-work.} While website accessibility has been extensively studied\cite{hackett2003accessibility, campoverde2023accessibility, mohammadi2024accessibility, agrawal2019evaluating, teixeira2021diversity, fok2022large, milne2014accessibility, ross2018examining}, to date, no comprehensive study has examined the accessibility of website ads at a large scale, leaving a significant gap in our understanding of website accessibility as a whole.
%the accessibility of web ads has never been investigated in depth. 
Only three studies have examined digital ad accessibility, focusing on small datasets of platform-specific ads and solely on blind website users. He et al.\cite{he2024tend} studied only 500 ad screens within Android apps and introduced a tool for detecting accessibility violations. Similarly, prior work manually examined {\tt alt text} on 67 websites \cite{thompson2001accessibility} and used a survey to understand screen reader users' challenges with website ads \cite{10.1145/3597503.3639229}. With the prevalence of website ads and their potential safety risks, the impact of website ads on accessibility remains an open yet important question.


\noindent {\bf Contributions.} In this paper, we conduct the first-of-its-kind large-scale, in-depth investigation of website ad accessibility and its impact on overall website accessibility. We perform an automated analysis of 430K website elements with nearly 100K website ad elements on the top 5K news and media websites. We first seek to understand the prevalence of inaccessible ads on the website and how they impact the overall accessibility of websites.
We build an automated pipeline to rigorously analyze the accessibility of website elements and the ads using IBM Equal Access Accessibility Checker and state-of-the-art ad-blocker, uBlockOrigin. Among ads that adversely impact a website's accessibility, we analyze the accessibility violations in accordance with WCAG guidelines. Identifying such violations provides key insights into commonly overlooked accessibility guidelines in ads and determines whether these violations are prevalent only in ads. To inform developers about accessibility violations across different ad-serving technologies, we further analyze inaccessible ads with respect to the technologies serving them.

Ads are historically more likely to lead to fraud, phishing, and scams~\cite{li2012knowing, rastogi2016these}. Even when ads are accessible, we investigate whether the provided accessible information truly represents the content and intent of the ad. We utilize open-source CLIP (Contrastive Language–Image Pretraining) model \cite{OpenAI-Clip} to confirm whether the content of ad images aligns with the provided alternative text for accessible ads. For instance, users with visual impairments solely rely on alternate text to access website content; false and misrepresented alternatives can mislead such users into involuntary interaction with ads. The onus for addressing inaccessible and misleading ads falls on the website developer whose website is hosting such ads.

% \todo{mention about manual study}
% \noindent {\bf  Methodology.} We build extend IBM Equal Access IBM Equal Access Accessibility Checker to  We utilize a top-of-the-line ad blocker, uBlock Origin, to remove ads and measure website's accessibility both with and without ads. We extract the violations specific to ad elements by differencing website's accessibility both with and without ads.
% % pinpointing which accessibility violation are connected to specific ad elements on the website is difficult. We employ XYZ to automatically analyze accessibility reports and identify violations specifically linked to advertisements. 
% Second, we utilize a combination of existing databases \cite{easylist, easyprivacy} containing known ad-serving technologies for labeling ad elements. 
% % 
% 
% % 
% This also involves verifying whether the alternative text correctly defines the ad or not.
% % 
% Lastly, we manually inspect the consequences of interacting with these misleading ads to determine whether they collect user identifiers for invasive tracking.

\noindent {\bf Findings.}
Our analysis reveals that 75\% of websites have ads that frequently fail to comply with WCAG guidelines. On average, we observe  11 more accessibility violations due to ads. 
% 
We further categorize the most common WCAG guideline violations found in ads to illustrate their potential impact on individuals with disabilities. We identified 28 different WCAG guideline violations in ad elements, with 7 of these violations predominantly occurring in only ad elements. These violations are related to missing captions, missing focus order, and missing page language, all of which are critical in ensuring smooth navigation on a website. 
% 
Our analysis also identifies the ad-serving technologies responsible for the majority of these violations. We found that 52\% of websites use one of Google's ad-serving technologies (e.g., DoubleClick), which account for over 14K violations in their ad elements.
% 

We show that the misrepresentation of data in alternate texts compared to the actual image deceives users with visual impairments and cognitive disabilities, making it difficult for them to interpret the intent of the ads. We found that 27\% of ad images misrepresent their content and intent. Furthermore, our manual inspection of ads from top-50 news websites reveals that up to 94\% of the ads collect trackable user identifiers upon {\tt onmouseover}, {\tt onhover}, and {\tt onclick}  events. These events help assistive technologies identify website elements that a user with disability desires to access. Thus, navigating ads can compromise the privacy of assistive technology users. To the best of our knowledge, this is the first work that investigates the accessibility violations of website ads on a large scale. 
% 

\noindent {\bf Data Availability:} Our data is available at \url{https://zenodo.org/records/13137429}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %\todo{Imp of Websites:} 
% About 15\% of the global population has some form of disability whose access to the internet depends on how accessible websites are. Many such users use assistive technologies like screen readers, which require highly accessible websites (e.g., properly labeled images) to function effectively~\cite{}. 
% %and include accessible digital content on websites is crucial 
% %Websites are essential in daily life, with millions available and billions of users relying on them ~\cite{?}. 
% % 
% %In practice, web developers often neglect accessibility when creating websites, leaving a significant portion of internet users in the dark.%: accessibility. 
% %% Therefore, it is essential for developers to ensure their websites are accessible to everyone, regardless of their abilities or preferred interaction methods.
% %% 
% %\todo{WCAG Guidelines:} 
% %Empirical studies show that accessibility issues are prevalent on real-world websites, leaving websites inaccessible for a significant portion of internet users. 
% %
% The Web Content Accessibility Guidelines (WCAG), led by the World Wide Web Consortium (W3C), have driven efforts to improve web accessibility.  As a result, numerous tooling and services test and improve the accessibility of websites today~\cite{}. 
% %
% While web accessibility is gradually improving due to these tools, the accessibility of {\em website advertisements} remains unexamined. 
% % 

% Web advertisements are the driving force behind free and open Internet, comprising nearly X\%  of the web content ~\cite{}. Web developers integrate ads on their webpage by leasing their website's space to ad technologies (e.g., Adsense~\cite{}) that serve user-relevant ads when a user visits a website.  Consequently, web developers give up control over what ad content will be served on their websites and if it will meet the WCAG accessibility guidelines. 

% Including ads on websites poses several accessibility challenges. First, popular web accessibility tools, like Google Lighthouse, do not include advertisements in their assessments, which overestimates accessibility scores. Second, the dynamic nature of ad content means website developers cannot predict which ads will be served to users, causing noticeable variation in accessibility scores. Therefore, even when a web developer makes the best effort to make the website WCAG complaint, ads can significantly deteriorate the overall accessibility score of the website. Third, inaccessible web advertisements cause additional problems for users with disabilities. As a result, users with disabilities are unable to access a significant portion of the website. This is especially alarming when ads pose privacy and security risks ~\cite{?}, as they are more likely to lead to fraud, phishing, and scams. Fourth, blanket blocked ads harm the free internet and cause fundamental equity issues by making ads completely unreachable. Accessible ads not only encourage free and open internet but also equip users with disabilities with the necessary context for safe and informed interaction with ads. 


% %  



% % %, security aspects ~\cite{?}, and user perceptions ~\cite{?}, but there is limited research on their impact on people with disabilities. 
% % % 

% % Evaluating the accessibility of advertisements on websites is challenging because 
% % % 
% % Another issue is that website developers often have limited control over the ads displayed, as they rely on ad-serving technologies like Taboola.
% % % 
% % This leaves manual checks as the primary method for assessing ad accessibility after deployment. 
% % % 
% % Additionally, the dynamic nature of ad content means website developers cannot predict which ads will be served to users, further complicating accessibility efforts.


 
% % State-of-the-art web accessibility tools, like Google Lighthouse, do not include advertisements in their assessments, resulting in incomplete accessibility scores. 









% %In the web ecosystem, websites have primarily two revenue-models: paid-subscriptions, advertisements, or a combination of both. 
% %  Advertisements have become an essential part of this ecosystem, forming a multi-billion-dollar market ~\cite{?}.




% %  Technology companies and organizations, led by initiatives from the World Wide Web Consortium (W3C), especially the Web Accessibility Initiative (WAI) and its Web Content Accessibility Guidelines (WCAG), are addressing these concerns to ensure web content is accessible.
% % 
% While web accessibility has been extensively studied~\cite{}, the accessibility of web ads has never been investigated in depth. Only three studies have investigated digital ad accessibility, however, on a very small dataset of platform-specific ads and for only blind web users. He et al.~\cite{?} studied only 500 ad screens within Android apps and introduced a tool for detecting accessibility issues. Similarly, prior work looked manually at only ALT tags of 67 websites ~\cite{}  and used a survey to understand screen reader users' challenges with web ads~\cite{}. With the prevalence of web advertisements and their potential safety risk, the impact of web ads on the accessibility of a website remains an open yet important question. 

% % Thompson and Wassmuth ~\cite{?} found that over half of the ads on 67 online newspaper websites lacked ALT tags.
% % Nengroo and Kuppusamy ~\cite{?} used questionnaires to assess but did not observe real-time interactions. 
% % 

% %%
% \todo{Our Work:} In this paper, we conduct the first large-scale, in-depth investigation on the accessibility of web ads and their impact on overall web accessibility. We perform an automated quantitative and qualitative analysis of nearly 100K web advertisement elements on the top 5000 news and media websites. We first seek to understand the prevalence of inaccessible ads on the web and how they impact the overall accessibility of websites.  
% Among those that adversely impact a website's accessibility score, we reason about the accessibility violations in accordance with the WCAG guidelines. Finding such violations provides key insight into commonly overlooked accessibility issues in ads and if and why they are prevalent only in ads. To inform developers about the accessibility issues with different ad-serving technologies, we further analyze the inaccessible ads with respect to the ad technologies serving them. Ads are historically more likely to lead to clickbait, fraud, phishing, and scams. Even when ads are accessible, we investigate if the provided accessible information truly represents the content and intent of the advertisements. For instance, users with visual impairments solely rely on such alternate descriptions to access web content; false and misrepresented alternates can mislead such users into involuntary interaction with ads. The onus of addressing inaccessible and misleading ads falls on the web developer whose website is hosting such ads.

% The first challenge is measuring precisely the accessibility of the ads, excluding the website's original elements. We utilize a top-of-the-line ad blocker called uBlockOrigin to remove advertisements and measure the webpage's accessibility both with and without ads. Another significant challenge involves pinpointing which accessibility issues are connected to which advertisement elements on the website. To address this, we employ XYZ to automatically analyze accessibility reports and identify violations specifically linked to advertisements. In order to determine the ad-serving technology, we utilize a combination of existing databases containing tracking URL lists and known hosting domains of ad technologies to trace the source of the ads. Finally, we utilize state-of-the-art open-source LLMs (Llama3) to confirm whether the content of ad images aligns with the provided alternative text for accessible ads. This also involves verifying whether the alternative text correctly identifies the ad as an advertisement. 



% %While previous studies on the accessibility of ads have been limited in scope and lack large-scale systematic research, our work addresses this gap with a comprehensive empirical


% %, both with and without advertisements, using an accessibility tool that accounts for ads.
% % 



==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/methodology.tex <==

\section{Research Questions}
Given the proliferation of ads on popular websites, their impact on vulnerable users, and the gap in developers' understanding of ad accessibility, we aim to answer the following research questions:
% 
\begin{enumerate}
    \item \textbf{RQ1:} How do advertisements impact the accessibility guideline violations of websites?
    \item \textbf{RQ2:} What are the most common accessibility guideline violations found in advertisements?
    \item \textbf{RQ3:} Which ad-serving technologies frequently exhibit accessibility violations in their served advertisements?
    \item \textbf{RQ4:} How is information misrepresented in the alternate text of advertisements?
\end{enumerate}

\section{Methodology}
\label{sec:methodology}
To address the research questions, we designed an automated pipeline to inspect websites, identify accessibility violations in each element, extract violations specific to ad elements, and categorize them based on WCAG guidelines \cite{WCAG-21}.
% To address the research questions, we designed an automated pipeline to inspect websites, identify accessibility violations in each element, extract violations in ad-slot elements, and categorize them based on Web Content Accessibility Guidelines (WCAG)\cite{WCAG-21}. 
% 
Figure \ref{fig:overview} illustrates the overview of the process used in our empirical investigation, which is completely automated and packaged into a single measurement tool. 
% 
\begin{table}[t]
\small
    \centering
    \scalebox{0.8}{\input{tables/sample-report}}
    % \vspace{0.2in}
    \caption{Sample accessibility evaluation report detailing elements and associated violation information.}
    \label{table:report}
    \vspace{-0.25in}
\end{table}
\subsection{Websites Visited}
%% 
We visit the top 5K news and media category websites from SimilarWeb \cite{Similar-web}, using a custom Selenium (version 4.11.2) based automated website navigator running on Google Chrome (version 120.0.6099.129).  
% 
Prior literature has also focused on this category of websites because they have the most ads \cite{thompson2001accessibility,zeng2020bad,he2024tend}, offering the most breadth and coverage of ads. 
% 
For every website, we launch our automated website navigator to first visit the website and then eventually trigger the accessibility evaluation using the IBM accessibility tool, as explained in Section~\ref{sec:accessiblity-evaluation}. 
%
It takes approximately 30 seconds for a website to fully load (until the onLoad event is fired), on average, and an additional five minutes to ensure all ads are loaded before applying the accessibility checks.  
% 
We use a stateless crawling process, with all cookies and local browser states cleared between consecutive visits. 
% 
This approach helps ensure that the collected accessibility data accurately reflects the current state of the website without being biased by previous visits. 
% 
We visited all 5K websites in North America. 
% 

We crawl each website twice to obtain two accessibility evaluation reports for the same website:
\begin{enumerate}
    \item $Report (R_{with-ads})$: Accessibility report of the website with ads.
    \item $Report (R_{without-ads})$: Accessibility report of the website without ads.
\end{enumerate}
% 
$Report (R_{with-ads})$ contains the accessibility report for all elements on the website, including ad elements.
% 
$Report (R_{without-ads})$ contains the accessibility report for all elements on the website, excluding ad elements.
% 
Finally, we extract the $ Report (R_{only-ads})$ by differencing the 
$R_{with-ads}$ and $R_{without-ads}$, which represents the accessibility report for the ad elements only:
\begin{equation}
    \underbrace{R_{with-ads}}_{\text{Website elements with Ads}} - \underbrace{R_{without-ads}}_{\text{Website elements without Ads}} = \underbrace{R_{only-ads}}_{\text{Ad elements}}
\end{equation}
% 
\noindent\textbf{Why do we need this approach to find the accessibility of ads?} To date, there does not exist any tool that can identify and isolate accessibility scores for ad elements alone. 
% 
Ads can only be evaluated post-deployment because, during the development phase, ad-serving technology only requires reserved space on the website. 
% 
The actual ads only appear on the website based on user client profiling and real-time advertiser bidding. 
% 
We opt to evaluate these ads post-deployment on the client side to understand the true accessibility impact of ads, offering insights for developers and ad-serving technologies. 

\begin{table}[t]
\small
    \centering
    \scalebox{0.85}{\input{tables/dataset}}
    % \vspace{0.2in}
    \caption{Number of website elements with violations during the campaign, detailing ad elements by violation level and criteria.}
    \label{table:dataset}
    \vspace{-0.25in}
\end{table}
%%
\subsection{Blocking Website Advertisements}
To measure the website's accessibility without ads, we aim to load the website without any ads in our crawler, which requires removing all ads before performing accessibility evaluations. 
% 
We leverage a widely used, advanced ad-blocking tool called uBlock Origin\cite{uBlock-origin} to remove ads from a website before it completely loads in the browser. 
% 
uBlock Origin relies on a crowd-sourced filter list\cite{easylist, easyprivacy}, which are databases of rules and patterns that identify and block resources from commonly used ad-serving technologies. 
% 
Almost all ad blocking tools\cite{uBlock-origin, Adblockplus, adguard} rely on the same filter lists and, therefore, have more or less similar effectiveness in blocking ads.  
% 
Internally, when a user visits a website, the ad blocker scans the page and its resources, comparing URLs and scripts against its filter lists.
% 
If it detects elements associated with ad-serving technology, it prevents these elements from being loaded on the page. 
% 
This can involve blocking requests to known ad servers, hiding ad elements within the DOM, or preventing ad scripts from executing. 
%
As a result, the ad content is not displayed to the user, resulting in an ad-free website, which we use to perform accessibility evaluations, $R_{without-ads}$. 
%
Prior work\cite{castell2022demystifying} on the effectiveness of ad-blocking tools has shown that uBlock Origin is the most effective ad blocker. 

%%
\subsection{Accessibility Evaluation}
\label{sec:accessiblity-evaluation}
After the website loads, we automatically perform a rigorous accessibility evaluation using the IBM Equal Access Accessibility Checker \cite{IBM-accessibility}, a Chrome extension. 
% 
Initially, we use Google's Lighthouse\cite{Google-lighthouse}, commonly used for quality checks during development. 
% 
However, tools like Lighthouse, Axe \cite{Axe}, and Wave \cite{Wave} exclude ad elements by default, leading to inaccurate measurements for sites with ads. 
% 
Thus, we use the IBM checker to assess accessibility for all website elements, including ads.
% After the website loads completely, we automatically perform rigorous accessibility evaluation of the website using the IBM Equal Access Accessibility Checker \cite{IBM-accessibility}, offered as a Chrome browser extension.
% % 
% Initially, we leverage Google's built-in accessibility tool, Lighthouse\cite{Google-lighthouse}, which is widely used by web developers to perform quality checks on websites while it is being developed. 
% % 
% Unfortunately, Lighthouse and several existing like Axe \cite{Axe}, and Wave \cite{Wave}, by default, exclude ad elements during the accessibility measurements of the website. 
% % 
% Using such tools to measure $R_{with-ads}$ leads to incorrect measurements for the accessibility of websites with ads. 
% % 
% Therefore, we choose the IBM accessibility checker to compute accessibility evaluation report for all website elements, including ads.
%%
Internally, IBM's accessibility checker injects a content script into the website to interact with the website's DOM. 
% 
The content script scans the website's DOM to identify elements and runs a series of checks based on the following predefined rules such as WCAG 2.1 \cite{WCAG-21}.
% 
The results are intercepted by our automated website navigator and stored in separate storage for downstream analysis. 
% 

%%
\noindent\textbf{Accessibility Report.} 
Table \ref{table:report} shows a sample accessibility evaluation report with a detailed analysis of violations, including page title, URL, HTML element type, element code, XPath, WCAG checkpoint, and violation level. Each checkpoint corresponds to a specific WCAG criterion with a description of the violation.
% Table \ref{table:report} shows a sample accessibility evaluation report.
% % 
% It includes a detailed analysis of accessibility violations found on a website's elements, including the page title, URL, HTML element type, element code, XPath, WCAG checkpoint, and WCAG violation level.
% % 
% Each WCAG checkpoint corresponds to a specific criterion within the WCAG levels and includes a description of the violation.
% 
The WCAG level indicates the priority and severity of accessibility violations, categorized into three levels:
% 
\begin{itemize}
    \item \textbf{Level A:} These guidelines are fundamental for all websites. Non-compliance makes website content inaccessible to users with disabilities. For example, text alternatives for non-text content (WCAG 1.1.1) are crucial for users with visual impairments. Meeting Level A criteria is a top priority. 
    % most fundamental web accessibility features that all Websites must include. Non-conformance to Level A makes website content completely inaccessible to users with disabilities.  For example, providing text alternatives for non-text content (WCAG 1.1.1) is essential for users with visual impairments who rely on screen readers. Meeting Level A success criteria for a website is of the highest priority. 
    \item \textbf{Level AA:} These guidelines should be met by most websites. Conformance to Level AA significantly improves the accessibility of website content. For example, ensuring that text and images of text have a contrast ratio of at least 4.5:1 (WCAG 1.4.3) is crucial for users with visual impairments, including those with color blindness.
    % Conformance to Level AA significantly improves the accessibility of web content. For example, ensuring that text and images of text have a contrast ratio of at least 4.5:1 (WCAG 1.4.3) is crucial for users with visual impairments, including those with color blindness.
    \item \textbf{Level AAA:} These guidelines represent the highest website accessibility standards for full accessibility. For example, sign language interpretation for pre-recorded audio (WCAG 1.2.6) benefits deaf users. Level AAA conformance is not mandatory for WCAG compliance as it applies to specific content types. \textit{Note: These violations require manual assessment and are excluded from this analysis}.
    
    % For example, providing sign language interpretation for all pre-recorded audio content in synchronized media (WCAG 1.2.6) benefits users who are deaf and rely on sign language. Level AAA conformance is not required for a website to be WCAG compliant, as the included accessibility features are only applicable to specific types of content. \textit{Note that these violations cannot be evaluated automatically and require manual assessment, thus they are excluded from this analysis.}
\end{itemize}
%  

%$R_{with-ads}$ and $R_{without-ads}$ ,

\noindent\textbf{Extracting Ad-elements.} We first generate the two accessibility reports of each website in our dataset, $R_{with-ads}$ and $R_{without-ads}$.
% 
$R_{with-ads}$ represents the accessibility report of all the website elements, including ads, as illustrated in Figure \ref{fig:overview} \ding{202} - \ding{205}.
% 
$R_{without-ads}$ represents the accessibility report of all the website elements excluding ads, as illustrated in Figure \ref{fig:overview} \ding{202} - \ding{203}.
%
Finally, we automatically compare the two accessibility reports by first matching website elements based on their code and Xpath location, resulting in a list of website elements that are not ads (\ding{202} and \ding{203}). 
% 
We exclude these elements from $R_{with-ads}$, which results in an accessibility report of ads only, $R_{ads-only}$ as illustrated in Figure \ref{fig:overview} \ding{204} - \ding{205}.
% On average, it took two minutes to generate an accessibility report for a single instance of a website.
% 
We analyzed 430K unique HTML elements with accessibility violations across 5k websites, of which 23.1\% are ad elements.
% 
Computing accessibility reports is time-consuming and resource-intensive due to the extensive checks required on the rendered page, styling, and HTML structure.
% Computing accessibility reports is compute-intensive and time-consuming due to the wide range of checks that the accessibility checkers have to perform on both the rendered page and the underlying styling and HTML structure. 
% 
It also cannot be deployed on the cloud, as certain accessibility metrics can only be measured when active display is available for UI rendering.
% 
Therefore, analysis on the 5K website consumed more than 484 CPU hours to generate accessibility reports spanning 20.6 GB.  
% 
Table \ref{table:dataset} lists the number of website elements with violations that we interacted with during this campaign.
% 
Specifically, it details the ad elements with violations, categorizing them by the level and criteria of violations.
%


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/related-work.tex <==
\section{Related Work}
\label{sec:related-work}

Accessibility of websites and mobile applications has been extensively studied \cite{hackett2003accessibility, campoverde2023accessibility, mohammadi2024accessibility, agrawal2019evaluating, teixeira2021diversity, fok2022large, milne2014accessibility, ross2018examining}. 
% 
Hackett et al. \cite{campoverde2023accessibility} used the Internet Archive’s Wayback Machine to demonstrate that websites have become progressively less accessible as their complexity has increased. 
% 
Teixeira et al. \cite{teixeira2021diversity} conducted a systematic literature review focusing on website accessibility within the tourism industry. 
% 
Similarly, Moreno et al. \cite{moreno2008guiding} proposed a method to improve website design for accessibility by addressing identified violations. 
% 
Fok et al. \cite{fok2022large} conducted a large-scale analysis of mobile applications to investigate how inaccessible user interfaces are. 
% 
Similarly, Milne et al. \cite{milne2014accessibility} and Ross et al. \cite{ross2018examining} found that missing or vague labels in mobile applications hinder screen readers from conveying information to visually impaired users.

%%
 Digital ads on websites and mobile applications are mainly studied for privacy-invasive targeted advertising mechanisms (\eg \cite{bashir2016tracing, englehardt2016online, eslami2018communicating}), malicious ads spreading malware or click fraud and phishing attacks (\eg \cite{li2012knowing, rastogi2016these}), and deceptive or manipulative content (\eg \cite{zeng2020bad}).
% 
However, there is very limited research specifically focused on the accessibility of online ads.
% 
He et al. \cite{he2024tend} conducted an empirical study on the accessibility of mobile ads for blind users in Android apps, identifying significant challenges such as missing {\tt alt text} for images, complex gestures problematic for screen readers, and ads that disrupt app functionality. 
% 
However, their analysis was limited to only 500 ad elements on mobile applications, so their insights are not applicable to website ads broadly.
% 
Similarly, Thompson et al. \cite{thompson2001accessibility} manually examined {\tt alt text} for ad elements on 67 news websites, while Chiou et al. \cite{10.1145/3597503.3639229} automatically detected reflow accessibility violations in website advertisements for keyboard users. Both studies are small-scale and on limited accessibility violations. 
% 
To date, the large-scale accessibility of website ads remains a significant and unresolved question.

%%
Several tools\cite{kumar2021comparing,gleason2020twitter,zhang2021screen, prakash2024all} have been developed to address accessibility issues. 
% 
Twitter A11y \cite{gleason2020twitter} is a browser extension designed to add alternative text to images on Twitter.
% 
Zhang et al. \cite{zhang2021screen} created a machine-learning model that infers accessibility metadata from mobile app screens, improving iOS VoiceOver functionality and enhancing accessibility for existing apps. 
% 
InstaFetch \cite{prakash2024all} is a browser extension that consolidates website content into a screen reader-friendly interface, allowing blind users to access information across multiple pages efficiently.
% 
while these tools may improve the accessibility of general website content, it is yet to be measured if these fully address the accessibility violation caused by the ads. 


%Studies done on mobile ads in Android Apps:

%[8] https://seal.ics.uci.edu/publications/2024_ICSE_AdMole.pdf

%[9] https://dl.acm.org/doi/pdf/10.1145/3491102.3502143

%[10] https://milnel2.github.io/files/mobileHealth.pdf

%[11] https://dl.acm.org/doi/pdf/10.1145/3234695.3236364

%[12] https://core.ac.uk/download/pdf/82110597.pdf

%These works focus on a range of accessibility concernss in Android apps, including labeling, touch target size, color contrast, and more:

%https://www.researchgate.net/publication/333625374_Accessibility_Assessment_in_Mobile_Applications_for_Android

%%https://ics.uci.edu/~iftekha/pdf/paper16.pdf

%https://www.researchgate.net/publication/333625374_Accessibility_Assessment_in_Mobile_Applications_for_Android

%https://ieeexplore.ieee.org/document/8918937

%https://www.researchgate.net/publication/317183694_Universal_Design_of_Mobile_Apps_Making_Weather_Information_Accessible

%https://dl.acm.org/doi/10.1145/3300176

%================================

% Works done on web accessibility



%[13] Literature review on University websites accessibility. 
%Link: https://link.springer.com/article/10.1007/s10209-021-00825-z

%[14] https://www.researchgate.net/profile/Gaurav-Agrawal-28/publication/332763704_Evaluating_Accessibility_and_usability_of_airline_websites/links/643e1aa02eca706c8b66a2ef/Evaluating-Accessibility-and-usability-of-airline-websites.pdf

%[15] This work analyzes prior studies done on educational websites accessibility. It analyzes 25 prior papers. 
%Link: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9092982

% [16] Power et al. found that only 50% of problems were addressed by the guidelines, revealing that meeting accessibility criteria does not ensure screen reader users have The Accessibility of Data Visualizations on the Web for Screen Reader Users access to the information. 
%Link: https://dl.acm.org/doi/10.1145/2207676.2207736

%Making memes accessibile
%Link: https://www.cs.cmu.edu/~jbigham/pubs/pdfs/2019/accessible-memes.pdf

%Accessibility in Visualization
%https://dl.acm.org/doi/abs/10.1145/3491102.3517630

%=================================

%Tools developed to improve accessibility

%Twitter: https://dl.acm.org/doi/abs/10.1145/3313831.3376728

%Mobile apps:
%https://dl.acm.org/doi/abs/10.1145/3411764.3445186



==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/results.tex <==
\section{Results}
\label{sec:results}
\begin{figure}
    \centering
    \include{plots/rq1-violations-diff}
    \vspace{-0.4in}
    \caption{CDF plot of websites by accessibility guideline violations in ad elements (\roa).}
    \label{fig:cdf-scores}
    \vspace{-0.2in}
\end{figure}
%
\begin{figure}
    \centering
    \include{plots/rq1-violations-histogram}
    \vspace{-0.4in}
    \caption{Histogram of the number of websites by accessibility guideline violations in ad elements (\roa).}
    \label{fig:histogram-violations}
    \vspace{-0.2in}
\end{figure}
\subsection{RQ1: Impact of Advertisements on Accessibility Violations}
We first examine the impact of ads on the number of accessibility violations on websites.
% 
This analysis demonstrates how third-party ad content can lower a website's accessibility, which has several downstream consequences, such as potentially low search rankings on Google due to accessibility violations\cite{Seo-accessibility} in addition to the fundamental inclusivity issues for users with disabilities. 
% 
Figure \ref{fig:cdf-scores} presents the cumulative distribution of websites and their WCAG guideline violations of ad elements (\roa). 
%The accessibility violations in websites with ads consistently stay on the right of the accessibility violations in websites without ads. 
% This shows that websites containing ads almost always incur more WCAG guidelines violations. 
% 
Concretely, the average violation count is 106.2, with a median of 72, for websites without ads (\rwoa). 
% 
For websites with ads (\rwa), the average violation count increases to 118.1, with a median of 81.
% , indicating a 10.1\% increase in violations when advertisements are present.
% 
Overall, the average violation count for ad elements (\roa) is to 11.7. 
% 
While the magnitude of the increase in violations may not look drastic, it is important to understand that a single violation directly points to an accessibility issue of a website element that makes it inaccessible for at least one type of disabled website user. 
% 
As mentioned before, WCAG guidelines violations in ads are more challenging to address than the violations in original website content, as a developer can immediately act on violations from original website content, whereas, in the case of ads, it is infeasible for the developer to address the violation due to user-specific dynamic nature of ads. 
%

To further understand the number of violations caused by the ads on websites, we distribute websites with the number of violations caused by ads. 
% 
Figure \ref{fig:histogram-violations} displays the distribution of websites for one or more accessibility guideline violations.  
% 
We find that nearly 74.6\% of websites have at least one accessibility violation in their ad elements (\roa), and 66.7\% of websites have an increase in violations after including ads (\rwoa $\rightarrow$ \rwa).
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, nearly 75\% of websites show at least one accessibility violation attributed to ad elements, underscoring the need for further investigation into these violations.
 }
\end{tcolorbox}

%%
\begin{table}[t]
\small
    \centering
    \scalebox{0.97}{\input{tables/rq2-violations}}
    \caption{Top-10 Most prevalent violations in ad elements}
    \label{table:rq2-violations}
    \vspace{-0.25in}
\end{table}
\begin{figure}[!t]
\vspace{0.1in}
\begin{subfigure}{.28\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq2-normal.png}
    \caption{Focus Visible}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
    \includegraphics[width=.90\linewidth,height=2cm]{images/rq2-ad.png}
    \caption{Focus Not Visible}
\end{subfigure}

\caption{The blue highlighted border shows the focus on the San Diego news block in (a), but it is not visible on the ad element in (b).} 
% \vspace{-3ex}
\label{fig:rq2-focus}
\vspace{-0.2in}
\end{figure} 
% 
\subsection{RQ2: Common Accessibility Violations in Advertisements}
To further understand the reason behind the increase in violations caused by the ad elements on websites, we investigate the different types of violations, when these violations occur, and how common those are in ad elements.  
\lstdefinestyle{base}{
language=html,
moredelim=**[is][\color{red}]{@}{@},
moredelim=**[is][\color{darkgreen}]{~}{~},
numbers=left,
numberstyle=\tiny,
stepnumber=1,
numbersep=5pt,
escapechar=`
}
\begin{lstlisting}[caption={The corresponding {\tt <a>} tag for the aforementioned sponsored ad does not comply with WCAG on input criteria.},language=html, label={lst:on-input}, style=base]
<a id="aw0" target="_blank" href="https://googleads.g.doubleclick.net/pcs/click?....." onfocus="ss('aw0')" onmousedown="st('aw0')" onmouseover="ss('aw0')" onclick="ha('aw0')">
        <img src="https://tpc.googlesyndication.com/simgad/2522640214132067527" border="0" width="292" height="30" alt="" class="img_ad">  
</a>
\end{lstlisting}
%%
\subsubsection{Prevalent Violations in Ad Elements (\roa)}
%
This analysis provides insights into design-specific violations within ad elements and their potential implications.
% 
Table \ref{table:rq2-violations} highlights the most prevalent violations we found in ads across 5K websites.
%
Note that these ad elements with violations are rendered at runtime, preventing developers from addressing them during deployment.

%% 
\noindent\textbf{Focus Visible} is one of the most common violations. Focus visible results enforce that keyboard focus indicators are visible when styling elements like links or ad elements using CSS. 
% 
In other words, website elements currently focused on should be highlighted. 
% 
For example, on the website {\tt 10news.com}, we identified a Google Ads iframe that violates this rule, as depicted in Figure \ref{fig:rq2-focus}(b). 
% 
In \ref{fig:rq2-focus}(a), the website developer has correctly implemented the focus visible feature by highlighting website cards with a blue border and thus adheres to focus visible. 
% 
Under WCAG Success Criterion 2.4.7 (Focus Visible)\cite{WCAG-list}, focus indicators must always be visible, which benefits users with motor disabilities, visual impairments (including low vision), cognitive disabilities, and those relying on accessibility tools like screen readers.
% 
We observe that 54.1\% of the website ad elements have not implemented focus visible.
%


% \vspace{-0.2in}
\begin{figure}[t]
    \centering
      \fbox{\includegraphics[width=0.40\textwidth]{images/rq2-on-input.png}}
      \begin{tikzpicture}[overlay]
          \fill[black] (-2.4,2.4) rectangle (-0.4,3.);
          \draw[red,thick,rounded corners] (-7.5,0) rectangle (-0.18,1.3);
    \end{tikzpicture}
        \caption{The Fox News weather widget, featuring a sponsored ad element highlighted in a red box, does not comply with WCAG on input criteria.}
        \label{fig:rq2-on-input}
        \vspace{-0.3in}
\end{figure}
% 

\begin{figure*}[!t]
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-captions}
    \vspace{-.4in}
    \caption{Missing Captions}
    \label{fig:normal}
\end{subfigure}
\hspace{-.2in} % Adjust horizontal space
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-focus-order}
    \vspace{-.4in}
    \caption{Focus-order}
    % \label{fig:lighthouse}
\end{subfigure}
\hspace{-.2in} % Adjust horizontal space
\begin{subfigure}{.33\textwidth}
    \include{plots/rq2-language}
    \vspace{-.4in}
    \caption{Language of Page}
    % \label{fig:noublock}
\end{subfigure}
\caption{Violations are predominantly found in ad elements (\roa) rather than in website elements (\rwoa).} 
\vspace{-4ex}
\label{fig:rq2-cdf}
\end{figure*}
%%
\noindent\textbf{In Input} is the second most common violation in ad elements that fails to inform users when their input action will change the context i.e., navigating to a different page or opening a new window. 
% 
This requirement is mandated by WCAG Success Criterion 3.2.2 (On Input) \cite{WCAG-list}. 
% 
According to this criterion, user actions on an interface component should not automatically change the context without prior notification. Violating "on input" causes confusion or disorientation from unexpected context changes.
% According to this criterion, any user action on an interface component should not automatically change the context unless the user has been informed of this behavior beforehand.
% % 
% Violating "on input" can significantly impact users with cognitive disabilities, leading to confusion or disorientation when unexpected context changes occur without prior notification.
% 
We observe this violation on 47.1\% of the websites' ad elements.
% 
For example, on the website {\tt foxnews.com}, we identified an ad that violates this rule, as shown in Figure \ref{fig:rq2-on-input}.
% 
The red-highlighted ad has associated {\tt onclick}, {\tt onmouseover}, {\tt onmousedown}, and {\tt onfocus} events, as shown in Listing \ref{lst:on-input}.
% 
These events open a new window (target="\_blank"), but there is no indication in the link text or an accessible tag like {\tt aria-label} to inform users that a new window will be opened. 
% 
It is mandatory to inform users about changes in context to prevent disorientation.
% 

% \begin{figure}[h]
%     \centering
    
%     % Subfigure 1: Image with overlay
%     \begin{subfigure}[b]{0.40\textwidth}
%         \centering
%         \fbox{\includegraphics[width=\textwidth]{images/rq2-on-input.png}}
%         \begin{tikzpicture}[overlay]
%             \draw[red,thick,rounded corners] (-3.2,0.6) rectangle (3.5,1.4);
%         \end{tikzpicture}
%         \caption{on-input-example}
%         \label{fig:rq2-on-input}
%     \end{subfigure}
%     \hfill
%     % Subfigure 2: Code listing
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \lstdefinestyle{base}{
%             language=html,
%             moredelim=**[is][\color{red}]{@}{@},
%             moredelim=**[is][\color{darkgreen}]{~}{~},
%             numbers=left,
%             numberstyle=\tiny,
%             stepnumber=1,
%             numbersep=5pt,
%             escapechar=`
%         }
%         \begin{lstlisting}[caption={On Input Example}, language=html, label={lst:on-input}, style=base]
% <a id="aw0" target="_blank" href="https://googleads.g.doubleclick.net/pcs/click?....." onfocus="ss('aw0')" onmousedown="st('aw0')" onmouseover="ss('aw0')" onclick="ha('aw0')">
%         <img src="https://tpc.googlesyndication.com/simgad/2522640214132067527" border="0" width="292" height="30" alt="" class="img_ad">  
% </a>
%         \end{lstlisting}
%     \end{subfigure}
    
%     \caption{Combined figure with image and code listing}
%     \label{fig:combined}
% \end{figure}
% 

%%
% \noindent\textbf{In Context} is the third most common violation by ad elements where hyperlinks do not provide link text, labels, or images with text alternatives. 
% % 
% This requirement is mandated by the WCAG Success Criterion 2.4.4 (Link Purpose - In Context)\cite{WCAG-list}. 
% % 
% According to this criterion, the purpose of each link should be clear from the link text alone or from the link text in conjunction with its context. 
% % 
% This is crucial for users who depend on screen readers to understand the purpose of each link without having to click on it first.
% % 
% We observed this violation in 38.3\% of the websites' ad elements. 
% % 
% For example, on the website {\tt mediapost.com}, we identified an ad by  Smart AdServer that violates this rule, as shown in Figure \ref{fig:rq2-in-context}. 
% % 
% The sponsored ad is rendered using an {\tt <a>} and {\tt <img>} tag without {\tt alt-text}, as shown in Listing \ref{lst:in-context}. 
% % 
% This forces users with disabilities to click on the link without knowing the outcome beforehand, which is particularly problematic if the link redirects to scam or phishing websites.
% \vspace{-0.1in}
% % 
% \begin{figure}[h]
%     \centering
%       \fbox{\includegraphics[width=0.40\textwidth]{images/rq2-alt-tag.png}}
%         \caption{The Mediapost website features a sponsored ad element that does not comply with WCAG in-context criteria.}
%         \label{fig:rq2-in-context}
%         \vspace{-0.2in}
% \end{figure}
% % 
% % 
% \lstdefinestyle{base}{
% language=html,
% moredelim=**[is][\color{red}]{@}{@},
% moredelim=**[is][\color{darkgreen}]{~}{~},
% numbers=left,
% numberstyle=\tiny,
% stepnumber=1,
% numbersep=5pt,
% escapechar=`
% }
% \begin{lstlisting}[caption={The corresponding {\tt <a>} tag for the aforementioned sponsored ad does not comply with WCAG in-context criteria.},language=html, label={lst:in-context}, style=base]
% <a href="https://use1.smartadserver.com/click?..." target="_blank">
%     <img id="img_36497925" src="https://creatives.sascdn.com/diff/1909/advertiser/522511/WBNR96-CausalIQ-001-728x90dbl_0046e903-e3e2-4c44-afc9-a1f30c6f8fe0.gif" width="728" border="0" height="90">
% </a>
% \end{lstlisting}
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, we observed 28 different types of violations, with the most prevalent being Focus Visible (54\%), and In Input (47\%) across various websites. 
    % and In Context (38\%) across various websites.
 }
\end{tcolorbox}

% 


\subsubsection{Violations in Ad Elements (\roa) vs. Non-ads Website Elements \rwoa}
% 
This analysis highlights the accessibility violations that are specific to ad elements (\roa) but not quite prevalent in non-ad elements (\rwoa). 
% 
We compare violations from over 99K ad elements and 331K non-ad elements.
% 
Figure \ref{fig:rq2-cdf}(a-c) shows the distribution of websites with the three most commonly found violations in ad elements (\roa), which are not common in non-ads website elements (\rwoa).

%%
\noindent\textbf{Missing Captions} (WCAG 1.2.4 \cite{WCAG-list}) is one of the most common accessibility violations found more in ad elements  (\roa) than standard website elements  (\rwoa). 
% from plots: 100-83.6 and 100-91.7 
% 
This criterion requires that pre-recorded and live audio content in synchronized media (such as videos) includes captions.
% 
Captions are essential for users who are deaf, as they provide a text alternative to spoken dialogue and important audio information.
% 
On average, 16.4\% of ad elements (\roa) contain at least one instance of this violation, whereas only 8.3\% of website elements (\rwoa) exhibit the same violation. 
% 
In other words, ad elements (\roa) are 2$\times$ more likely to be missing captions than non-ads elements (\rwoa) on websites.

%%
\noindent\textbf{Focus Order} (WCAG 2.4.3 \cite{WCAG-list}) is found to be more prevalent in ad elements (\roa) than non-ads website elements (\rwoa).  
% from plots: 100-72.9 and 100-80.9
This criterion requires that the navigation order of interactive elements on a website is logical and intuitive, ensuring users can navigate through content in a predictable manner. 
% 
Proper focus order is crucial for users who rely on keyboard navigation, such as individuals with motor impairments or those using assistive technologies like screen readers. 
% 
Without a logical focus order, users may struggle to understand the structure of the page, miss important information, or find it difficult to interact with the content. 
%
On average, 27.1\% of ad elements (\roa) contain at least one instance of this violation, whereas only 19.1\% of website elements (\rwoa) exhibit the same violation.

%%
\noindent\textbf{Language of Page}  (WCAG 3.1.1 \cite{WCAG-list}) is another accessibility violation that is found more in ad elements than non-ad website elements. 
% 
This criterion requires that the primary language of a website element is clearly defined in the HTML. 
% 
Declaring the language is essential for users who rely on assistive technologies, such as screen readers, which use this information to provide accurate pronunciation and interpretation of the content. 
% 
Without the language of the page specified, users with visual impairments or cognitive disabilities may have difficulty understanding the content, leading to a less accessible and non-inclusive website experience. 
% from plots: 100-54.7 and 100-79.9 
On average, 45.3\% of ad elements (\roa) contain at least one instance of this violation, whereas only 2.1\% of website elements (\rwoa) exhibit the same violation.  
% 
Thus, ad elements (\roa) are 21$\times$ more likely to have this violation than non-ad elements (\rwoa).  
% 45.23/2.1
This significant difference points to the special ad accessibility case where website developers are not able to enforce language constraints on the ads served on their website due to the user-specific and dynamic nature of websites.  
% checkpoint.xlsx
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, we observed seven violations more common in ad elements (\roa) than in website elements (\rwoa): missing captions, incorrect focus order, undefined page language, insufficient text spacing, hover content violations, keyboard accessibility issues, and focus-related violations.
 }
\end{tcolorbox}


%%
\begin{table*}[t]
\small
    \centering
    \scalebox{0.9}{\input{tables/rq3-adv-violations}}
    % \vspace{0.2in}
    \caption{Top five ad-serving technologies with the highest number of violations.}
    \label{table:rq3-adv-violations}
    \vspace{-0.25in}
\end{table*}
%
\subsection{RQ3: Most Prevalent Ad-Serving Technologies on Websites with Ad Serving Violations}
We investigate the ad-serving technologies that deliver ads on websites with the most accessibility violations. 
% 
This analysis aims to guide website developers in selecting ad-serving technologies that comply with WCAG guidelines. 
% 
Additionally, it encourages ad-serving technologies to prioritize accessibility considerations before delivering ads on websites.
% 
Table \ref{table:rq3-adv-violations} lists the top ad-serving technologies prevalent on websites with the highest number of violations in ad elements (\roa). 

%%
\noindent\textbf{Taboola}  is a content discovery platform that promotes personalized content recommendations across websites. 
% 
In our investigation, it is found on 8.2\% of the inspected websites with a total of 18K violations.
% 
Common ad violation is related to guideline 1.1.1 \cite{WCAG-list}, which mandates that all content must have a text alternative for non-text content, found in 5,699 ads.
% 
Another common violation is related to guideline 3.2.2 \cite{WCAG-list}, which mandates providing adequate feedback when an action opens a new window or changes the context.
% 
This guideline is violated in 5,057 ads. 
% 
Lastly, guideline 2.4.7 \cite{WCAG-list}, which requires visible focus indicators for interface components to assist users navigating with keyboards or alternative devices, is violated in 4,658 ads served by Taboola.

%%
\noindent\textbf{DoubleClick} 
%The first two most prevalent ad-serving technologies are owned by Google.
% 
is Google's ad management platform, optimizing digital ad campaigns. 
% 
In our investigation, it is found on 31.5\% of inspected websites with a total of 10K violations.
% 
Common ad violations include not informing users when their input action will open a new window or change context (Guideline 3.2.2) \cite{WCAG-list}, which is found in 3,369 ads.
% 
Another common DoubleClick violation is related to guideline 2.4.4 \cite{WCAG-list}, which ensures links have clear, context-independent purposes,  benefiting screen reader users. 
% 
This guideline is violated in 3,344 ads.
% 
Lastly, Guideline 2.4.7 \cite{WCAG-list} mandates visible focus indicators for interface components, aiding users navigating with keyboards or alternative devices, and is violated in 1,675 ads served by DoubleClick.

%%
\noindent\textbf{RevContent} is an ad-serving technology that delivers personalized ad recommendations across various websites. 
% 
In our investigation, it is found on 6.5\% of inspected websites with a total of 3K violations.
% 
Common ad violations include not informing users when their input action will open a new window or change context (Guideline 3.2.2) \cite{WCAG-list}, which is found in 1,375 ads.
% 
Another common violation is related to guideline 2.4.1 \cite{WCAG-list}, which ensures that all functionality is accessible from a keyboard.
% 
This guideline is violated in 1,113 ads.
% 
Additionally, guideline 1.2.1 \cite{WCAG-list}, which requires that all multimedia content has a synchronized captioning or a transcript, is violated in 232 ads served by RevContent.

% \noindent\textbf{Google Syndication} is found on 20.4\% of websites.
% % 
% Common ad violations include failing to meet Guideline 2.4.7, which mandates visible focus indicators for interface components, found in 1,844 ads.
% % 
% Guideline 1.1.1 mandates that all non-text content (e.g., images) have text alternatives that convey their purpose. 410 ads served by syndication violate this guideline.
% % 
% Guideline 4.1.2 ensures that interactive elements are programmatically determinable for users relying on assistive technologies, and it is violated in 25 ads.

%%
% \noindent\textbf{OpenX}  is an advertising technology company that operates a real-time bidding platform for digital advertising. 9.4\% of websites contain ads served by OpenX.
% % 
% Common ad violations include failing to meet Guideline 2.4.1, which ensures direct access to primary content for sequential navigation, found in 668 ads.
% % 
% Guideline 2.4.7 mandates visible focus indicators, which was violated in 118 ads.
% % 

% \gulzar{Can we add taboola as well since it has the most violations?}
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, 52\% of websites using Google's ad-serving technologies violate WCAG guidelines across over 14K ad elements. Taboola serves the most ad elements with accessibility violations.
 }
\end{tcolorbox}

%%
\subsection{Misrepresentation of Alt Text in Advertisements}
\label{sec:misrepesentation}
Among the ads that do not lead to accessibility violation, we investigate the accessible information associated with ads that truly represents the intext and content of the ad. 
% 
Prior work privacy implications of ads~\cite{book2013longitudinal, book2015empirical, Alrizah19IMCerrorsMisunderstandings,Le21anticvndss,Bashir:2018:TCC:3278532.3278573} and malvertising~\cite{sood2011malvertising, xing2015understanding, arrate2020malvertising} show that clickbait~\cite{li2024attention,ahmad2024review} and false ads~\cite{handler1929false} can lead to scams, phishing, and fraud.  
% 
Analyzing alternate texts of otherwise accessible ads is important because it highlights how effective alternate texts are in effectively conveying the content of ads to users with disabilities.

%%
We start by extracting {\tt <img>} tags with alt text from the ads' HTML and collecting their {\tt src} values, which contain the image URLs. Next, we use the CLIP (Contrastive Language–Image Pretraining) model~\cite{OpenAI-Clip} to assess the relevance between images and their alt text. CLIP encodes images and text into a shared embedding space, allowing us to compute the cosine similarity between them. We classify alt text as redundant if the cosine similarity is below 0.5, which is the optimal threshold reported in previous research \cite{ahmad2024scs}. This approach efficiently evaluates the semantic alignment between visual and textual data.
% We start by extracting {\tt <img>} tags with alt text from the ads's HTML and collecting their {\tt src} values, which contain the URLs of the loaded images. 
% % We then compare these URLs against EasyList, a widely used database of tracking urls maintained by most ad blockers. 
% % If a URL appears in EasyList, it is identified as an advertisement.
% % 
% Next, we use the CLIP (Contrastive Language–Image Pretraining) model~\cite{OpenAI-Clip} to assess the relevance between images and their textual descriptions. 
% % 
% CLIP encodes both images and text into a shared embedding space, allowing us to compute the cosine similarity between these embeddings.
% % 
% We determine the relevance of the alt text to the image based on this similarity score. 
% % 
% Specifically, if the cosine similarity is below 0.5, we classify the alt text as redundant with respect to the image. 
% % 
% The cosine similarity threshold of 0.5 is previously reported to be the optimal threshold \cite{ahmad2024scs}. 
% % 
% This approach provides a robust and efficient means to evaluate the semantic alignment between visual and textual data.

%%
Overall, across 5K websites,  we find 9,827 ad images with alt text.
% 2665/9827
Of these, 27.1\% of ads have a cosine similarity score below 0.5, indicating a low level of similarity between the text and the ad image.
% 
For example, Figure \ref{fig:rq5-misrepresentation}(a) shows an image of shoes on a bench, served by Taboola on {\tt wsfa.com}, but the alt text describes foxes stealing footwear. This alt text mimics a news headline to confuse users, with a cosine similarity score of 0.33.
% 
Similarly, Figure \ref{fig:rq5-misrepresentation}(b) shows a hotel image on {\tt clickorlando.com}, but the alt text describes hotels turned into apartments for affordable housing. This alt text also resembles a news headline,  with a cosine similarity score of 0.28.
% For example, Figure \ref{fig:rq5-misrepresentation}(a) shows an image of several pairs of shoes placed on a bench, which is an ad served by Taboola Ad-serving technology on {\tt wsfa.com}. 
% % 
% However, its alt text describes a story about "foxes accused of stealing crocs and sandals from campers, after many pairs were found at a den". 
% % 
% The alt text is intentionally designed to mimic a news headline in order to confuse users visiting news websites.
% % 
% The image and the alt text have a cosine similarity score of 0.33, indicating a significant mismatch.
% % 
% Similarly, Figure \ref{fig:rq5-misrepresentation}(b) shows an image of a hotel, but the alt text describes distressed hotels turned into apartments for affordable housing on {\tt clickorlando.com}.
% % 
% Again, the alt text mimics a news headline in order to confuse users visiting news websites.
% % 
% The image and the alt text have a cosine similarity score of 0.28, indicating a significant mismatch.
% 
The alt texts of these ads do not disclose that they are ads and not the content served by the website. 
% They are often presented as news stories to deceive users, making them appear as legitimate content. 
% This can be especially problematic on news websites, where users expect genuine news stories, not advertisements masquerading as such. 
% 
Users may only realize it is an ad after performing actions like pressing enter to open the link, only to be redirected to a page outside the original domain. 
% 
Malicious and false ads represented as news in alt text can redirect to scam and phishing websites, compromising the safety of users with disabilities who struggle to assess a website's trustworthiness. 
%
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} Overall, 27\% of the nearly 10K ads have alt text that misrepresents ad image's content and intent.
 }
\end{tcolorbox}
% 
\begin{figure}[!t]
\vspace{0.1in}
\begin{subfigure}{.23\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq5-taboola.png}
    \caption{Alt-text: Foxes accused of stealing Crocs, sandals from campers after many pairs found at den.}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
    \includegraphics[width=.99\linewidth, height=2cm]{images/rq5-cloudnary.png}
    \caption{Alt-text: Distressed hotels turned into apartments for affordable housing.}
\end{subfigure}

\caption{Misrepresentation of alt-text in image tags of ads.} 
\vspace{-0.3in}
\label{fig:rq5-misrepresentation}
\end{figure} 

%%
%% Privacy implication of having inaccessible ads
\noindent\textbf{Privacy implication of misleading advertisements.} We manually inspect the consequences of interacting with these misleading ads to determine if any user identifiers are collected for invasive tracking {\tt onhover}, {\tt onmouseover}, or when the user presses enter (for tabbable access) on these ads. 
% 
These three events are key resources for assistive technologies like screen readers to collect accessible information from website elements and deliver it to users using them  


% 
Prior research has shown that network traffic resulting from interacting with ads may contain user identifiers in headers \cite{rieder2024beyond, bujlow2015web}, cookies \cite{munir2023cookiegraph, amjad2024blocking}, and parameters \cite{munir2023purl}. 
% 
These identifiers can be used to trace a user's browsing activity on the web, violating their privacy. 
%Although these identifiers are encrypted, popular 
Lists maintained by ad-blockers identify specific headers\cite{Headers}, cookies\cite{CookieList}, and parameters\cite{AdguardBlockParam} as tracking identifiers for users. 
% 
We compare our network traffic from manually interacting with ads on the top 50 news websites against these lists to identify any tracking of user identifiers. 
% 
Our results show that on 94\% of websites, at least one tracking identifier is sent to an external server by hovering, and on 98\% of websites, at least one tracking identifier is sent to an external server by pressing enter on the ads. 
% 
Both events are essential actions that screen readers perform to read and announce website elements' content. None of the actions are necessary to access ads for regular users. 
%On hover, we do not find any trackable user identifiers transmitted through cookies and headers, but 84 different query parameters are sent to external servers. 
%In contrast, when pressing enter, 340 cookies, 12 headers, and 865 different query parameters are identified as trackable user identifiers using the lists.
% 
\begin{tcolorbox}[colback=blue!5!white]
 {
    {\bf \em Finding.} On 94\% of websites, hovering sends tracking data to external servers, forcing users with disabilities to compromise privacy to navigate ad content, unlike regular users.
 }
\end{tcolorbox}

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/parts/validitiy.tex <==
% \vspace{-0.15in}
\section{Threat to validity}
\label{sec:validity}
% 
\noindent\textbf{Internal validity.}
Our analysis in Section~\ref{sec:results} involves collecting ad elements (\roa) by differencing website elements without ads (\rwoa) from those with ads (\rwa). 
% 
However, various confounding factors may influence \roa.
% 
For instance, some websites dynamically fetch different elements, including ads, on each visit.
% 
Consequently, website elements loaded in \rwa might not appear in \rwoa. 
% 
Other factors include changes in behavior due to the environment (\eg browser and host OS), visit time, and location.
% 
To minimize this threat, we perform the two visits in quick succession and maintain consistent environments across different states, ensuring the same location, browser, and stateless crawls.

%%
\noindent\textbf{External validity.} 
% 
The IBM Equal Access Accessibility Checker \cite{IBM-accessibility} on different browsers might produce different accessibility violations due to the browser's built-in features, such as Safari's default blocking of certain ad-serving technologies \cite{Safari-ITP}. 
% 
We conduct our experiments using the Chrome browser with a Chrome-based extension, which is the most widely used browser, to minimize this threat.

%%
\noindent\textbf{Construct validity.}
We collect the website's elements at page load time and do not capture changes in accessibility violations triggered by user interactions such as scrolling and clicking. This is a general limitation of dynamic analysis that is challenging to overcome due to the numerous navigation and interaction scenarios on websites. 

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/tables/clauses.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{3.5cm}|>{\raggedright\arraybackslash}p{10cm}|}
\hline
\textbf{Clause} & \textbf{Text} \\
\hline
1.1.1 & Non-text Content \\
1.1.1 & Non-text Content; 4.1.2 Name, Role, Value \\
1.2.1 & Audio-only and Video-only (Prerecorded); 1.2.2 Captions (Prerecorded); 1.2.4 Captions (Live) \\
1.3.1 & Info and Relationships \\
1.3.1 & Info and Relationships; 4.1.2 Name, Role, Value \\
1.3.1 & Info and Relationships; 3.3.2 Labels or Instructions \\
1.3.2 & Meaningful Sequence \\
1.3.3 & Sensory Characteristics \\
1.3.5 & Identify Input Purpose \\
1.4.1 & Use of Color \\
1.4.3 & Contrast (Minimum) \\
1.4.4 & Resize text \\
1.4.12 & Text Spacing \\
1.4.13 & Content on Hover or Focus \\
2.1.1 & Keyboard \\
2.1.1 & Keyboard; 2.4.3 Focus Order \\
2.1.2 & No Keyboard Trap \\
2.2.1 & Timing Adjustable \\
2.4.1 & Bypass Blocks \\
2.4.2 & Page Titled \\
2.4.4 & Link Purpose (In Context); 4.1.2 Name, Role, Value \\
2.4.6 & Headings and Labels \\
2.4.7 & Focus Visible \\
2.4.7 & Focus Visible; 3.2.1 On Focus \\
2.5.3 & Label in Name \\
3.1.1 & Language of Page \\
3.2.1 & On Focus \\
3.2.2 & On Input \\
3.3.2 & Labels or Instructions \\
4.1.2 & Name, Role, Value \\
\hline
\end{tabular}


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/tables/dataset.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{1.2cm}|>{\raggedright\arraybackslash}p{1cm}|>{\raggedright\arraybackslash}p{4.9cm}|>{\raggedleft\arraybackslash}p{1cm}|}
     \cline{1-4}
     {\bf Violation } & {\bf Element} & {\bf WCAG} & {\bf Count}\\ 
     \cline{1-4}
        \multirow{2}{*}{Overall} & All & - & 430,497 \\
                  & Ad & - & 99,422 \\
        \cline{1-4}
        \multirow{3}{*}{Levels} & \multirow{3}{*}{Ad} & A  & 80,220 \\
                &  & AA  & 43,591 \\
                
        \hline
        \multirow{30}{*}{Criterion} & \multirow{30}{*}{Ad} & 2.4.7 Focus Visible& 41,110 \\ &  & 2.4.1 Bypass Blocks& 37,357 \\ 

                &  & 3.2.2 On Input & 26,629 \\
                & & 1.1.1 Non-text Content& 16,387 \\
                &  & 4.1.2 Name, Role, Value& 15,712 \\
                &  & 2.4.4 Link Purpose (In Context)& 7,714 \\
                &  & 1.3.4 Orientation& 6,493 \\
                &  & 1.3.1 Info and Relationships& 6,118 \\
                &  & 2.1.1 Keyboard& 6,026 \\
                &  & 2.4.3 Focus Order& 3,575 \\
                &  & 1.4.3 Contrast (Minimum)& 2,890 \\
                &  & 2.5.3 Label in Name& 1,190 \\
                &  & 1.2.1 Audio-only and Video-only& 1,147 \\
                &  & 1.2.4 Captions (Live)& 1,144 \\
                &  & 1.4.1 Use of Color& 1,021 \\
                &  & 3.3.2 Labels or Instructions& 269 \\
                &  & 1.3.3 Sensory Characteristics& 92 \\
                &  & 3.1.1 Language of Page& 60 \\
                &  & 1.4.12 Text Spacing & 26 \\
                &  & 1.4.4 Resize text& 21 \\
                &  & 2.1.2 No Keyboard Trap& 17 \\
                &  & 3.2.1 On Focus& 13 \\
                &  & 2.4.2 Page Titled& 6 \\
                &  & 2.4.6 Headings and Labels& 6 \\


                
                &  & 1.3.2 Meaningful Sequence& 3 \\
                
                
                &  & 1.3.5 Identify Input Purpose& 2 \\
                &  & 2.2.1 Timing Adjustable & 2\\
                &  & 1.4.13 Content on Hover& 1 \\
                

                
     \cline{1-4}
\end{tabular}

==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/tables/methodology-example_report.tex <==
\begin{tabular}{|p{1.5cm}|p{6.8cm}|}
\hline
\textbf{Feature} & \textbf{Example} \\
\hline
Page title & Atlanta news, Georgia news, Breaking news from The Atlanta Journal-Constitution - AJC.com \\
\hline
Page URL & \url{https://www.ajc.com/} \\
\hline
Scan Label & scan\_1 \\
\hline
Issue ID & 2748300732 \\
\hline
Issue Type & Violation \\
\hline
Toolkit level & 1 \\
\hline
Checkpoint & 1.1.1 Non-text Content \\
\hline
WCAG level & A \\
\hline
Rule & img\_alt\_valid \\
\hline
Issue & The image has neither an accessible name nor is marked as decorative or redundant \\
\hline
Element & img \\
\hline
Code & \texttt{<img style="display: block; padding: 0px; margin: 0px; border-width: 0px; min-width: 0px; min-height: 0px; max-width: none; max-height: none; -webkit-tap-highlight-color: rgba(0, 0, 0, 0); user-select: none; box-sizing: content-box; height: 100\%; width: 100\%; top: 0px; left: 0px; position: absolute;" src="https://clipcentric-a.akamaihd.net/file/1846203/master/1720505441/RhmEzmzh?f=auto" draggable="false">} \\
\hline
\end{tabular}


==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/tables/rq2-violations.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{6.8cm}|>{\raggedright\arraybackslash}p{1.2cm}|}
\hline
\textbf{Violation in Ad elements (\roa) } & \textbf{Websites} \\
\hline
Check the keyboard focus indicator is visible when using CSS declaration for 'border' or 'outline' & 2,708 \\
\hline
Inform the user when their input action will open a new window or otherwise change their context & 2,358 \\
\hline
 Hyperlink has no link text, label or image with a text alternative & 1,915 \\
\hline
 Verify \texttt{<frame>} content is accessible & 1,808 \\
\hline
Confirm the element should be tabbable and if so, it becomes visible when it has keyboard focus & 1,632 \\
\hline
Content is not within a landmark element & 1,605 \\
\hline
Verify there is a way to bypass blocks of content that are repeated on multiple Web pages & 1,490 \\
\hline
Confirm Windows high contrast mode is supported when using CSS to include, position or alter non-decorative content & 1,427 \\
\hline
Page detected as HTML, but does not have a 'lang' attribute & 1,374 \\
\hline
Inline frame does not have a 'title' attribute & 1,310 \\
\hline
\end{tabular}



==> ISCE_-_Accessibility_Issues_in_Ad-Driven_Web_Applications__2_/tables/rq3-adv-violations.tex <==
\begin{tabularx}{\textwidth}{|p{1.8cm}|p{1.4cm}|l|l|l|X|l|}
    \hline
    \textbf{Domain} & \textbf{Company} & \textbf{Websites}& \textbf{Violations} & \textbf{WCAG } & \textbf{Description} & \textbf{Count} \\
    \hline
    \multirow{3}{*}{taboola.com} & \multirow{3}{*}{Taboola} & \multirow{3}{*}{411}& \multirow{3}{*}{17,522} & 1.1.1  & All non-text content have text alternatives to ensure accessibility for users who rely on assistive technologies. & 5,699 \\
    \cline{5-7}
    &&&& 3.2.2  & User inputs should not trigger unexpected changes or disruptions in content. &  5,057 \\
    \cline{5-7}
    &&&& 2.4.7& Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 4,658\\
    \hline
    \multirow{3}{*}{doubleclick.net} & \multirow{3}{*}{Google} & \multirow{3}{*}{1,577} & \multirow{3}{*}{10,108}& 3.2.2  & User inputs should not trigger unexpected changes or disruptions in content. & 3,369 \\
    \cline{5-7}
    &&&& 2.4.4  & The purpose of a link is clear from its context, ensuring users understand where the link will take them. & 3,344 \\
    \cline{5-7}
    &&&& 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 1,675\\
    \hline
    
    %%
    \multirow{3}{*}{revcontent.com} & \multirow{3}{*}{RevContent} & \multirow{3}{*}{325}& \multirow{3}{*}{3,204} & 3.2.2 & User inputs should not trigger unexpected changes or disruptions in content. & 1,375 \\
    \cline{5-7}
    &&&& 2.4.1  & Users can bypass repetitive content, such as navigation menus, to access the main content more efficiently. & 1,113\\
    \cline{5-7}
    &&&& 1.2.1  & Text alternatives/captions for prerecorded audio and video content. & 232\\
    \hline
    %%
    \multirow{3}{*}{\parbox{1.5cm}{googlesyndica\\tion.com}} & \multirow{3}{*}{Google} & \multirow{3}{*}{1,021}& \multirow{3}{*}{2,339} & 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 1,844 \\
    \cline{5-7}
    &&&& 1.1.1 & All non-text content have text alternatives to ensure accessibility for users who rely on assistive technologies. &  410 \\
    \cline{5-7}
    &&&& 4.1.2  &  User interface elements have proper names, roles, and values to ensure they are accessible and understandable by assistive technologies. & 25\\
    \cline{5-7}
    \hline
    %%
    \multirow{3}{*}{google.com} & \multirow{3}{*}{Google} & \multirow{3}{*}{365}& \multirow{3}{*}{2,209} & 3.2.2 & User inputs should not trigger unexpected changes or disruptions in content. & 569 \\
    \cline{5-7}
    &&&& 4.1.2 &  User interface elements have proper names, roles, and values to ensure they are accessible and understandable by assistive technologies. &  516 \\
    \cline{5-7}
    &&&& 2.4.7  & Any interactive element has a visible indicator of focus to help users navigate and interact with content. & 504\\
    \cline{5-7}
    \hline
\end{tabularx}

==> parts/citations.tex <==
\begin{thebibliography}{00}

\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.









\end{thebibliography}

==> parts/graveyard.tex <==
In this section, we describe the design and implementation details of our accessibility report collection pipeline. Our crawling infrastructure, based on a campus network in North America, comprised of a ??-node cluster with ?? cores at ??GHz, ??GB storage, and ??GB memory. Figure X provides an overview of the pipeline, which starts with automated website crawling using the Selenium web driver and using \textbf{IBM EEAC} chrome extension that generates accessibility reports for web pages. The features that the accessibility report gets, along with an example is shown in table ??. We first run this script on top 5k news websites, first without \textbf{uBlock Origin} chrome extension and then with the extension enabled. We get two accessibility reports for each website and then using those reports we compute the difference between the two on the basis of "Code" to identify violations that were introduced due to ads. We combine all the files containing the differences to form a single data frame on which further analysis is performed.

\subsection{Selenium Script}
The Selenium script automates accessibility testing of websites using the IBM EAAC extension in Chrome. It reads URLs from a text file and processes each to download and save the HTML content, both with and without the adblocker. The script configures a Chrome WebDriver with options to load the IBM accessibility extension and optionally the adblocker. It navigates to each website, interacts with the extension through DevTools, and saves the accessibility report, first with and then without the adblocker enabled, to a designated directory. We generate accessibility reports on landing pages of top 5k news websites using the IBM EAAC extension. We give a delay of 10 seconds on each web page to make sure the page is completely loaded and the browser window is opened in maximized mode. There is another 3 second delay to make sure DevTools is open and the extension is ready. Upon triggering the IBM EAAC extension, an additional delay of 20 seconds is introduced to ensure the complete execution of the extension. Finally, the reports are saved in a designated directory in xlsx format. If a URL causes an error, the process terminates, and the URL is marked as crashed.

\subsection{IBM EAAC Extension}
The IBM Easy Accessibility Extension (EAAC) enables users to generate accessibility reports for web pages. Once activated in a Chrome browser session, the extension conducts real-time analysis of webpage accessibility. It examines critical elements like color contrast, text size, and semantic structure to verify adherence to accessibility standards. When integrated with DevTools, the extension delivers precise insights into potential accessibility issues that require manual review, recommendations for enhancement and identification of accessibility violations. Users can interact with the extension to explore the accessibility report, which features actionable insights and highlighted areas requiring attention. The issues are categorized in following levels:
\begin{itemize}
    \item \textbf{Level 1 -} The most essential issues to address
    \item \textbf{Level 2 -} The next most important issues
    \item \textbf{Level 3 -} Necessary to meet requirements
    \item \textbf{Level 4 -} Further recommended improvements to accessibility
\end{itemize}
We used IBM EAAC Extension because not only it was including ads while generating the accessibility report but it could be easily integrated with chrome Devtools and provided a detailed accessibility report. 
\subsection{uBlock Origin Extension}
uBlock Origin is a widely acclaimed browser extension renowned for its robust ad-blocking capabilities. Developed as an open-source project, uBlock Origin operates by leveraging filter lists—lists of rules that dictate what elements (such as advertisements, trackers, and other undesirable content) should be blocked on web pages.  When a user visits a web page, uBlock Origin parses these filter lists and applies rules to decide which elements to block or allow based on their URLs and other criteria. This process occurs in real-time as the page loads, ensuring that unwanted content such as ads and tracking scripts are intercepted before they can display or execute.
\subsection{Dataset}
We generate accessibility reports for top 5k news websites. We only consider 2608 since these include both the versions of the accessibility report, with and without ad block. If either version is absent due to any reason, we skip that website. We get the difference between the two versions of the reports to get the issues that were exclusively present in the version without an ad blocker. There was a total of 164,306 issues of which 54,610 were violations, 32,345 were recommendations and 77,351 required review.

==> tables/clauses.tex <==
\begin{tabular}{|>{\raggedright\arraybackslash}p{3.5cm}|>{\raggedright\arraybackslash}p{10cm}|}
\hline
\textbf{Clause} & \textbf{Text} \\
\hline
1.1.1 & Non-text Content \\
1.1.1 & Non-text Content; 4.1.2 Name, Role, Value \\
1.2.1 & Audio-only and Video-only (Prerecorded); 1.2.2 Captions (Prerecorded); 1.2.4 Captions (Live) \\
1.3.1 & Info and Relationships \\
1.3.1 & Info and Relationships; 4.1.2 Name, Role, Value \\
1.3.1 & Info and Relationships; 3.3.2 Labels or Instructions \\
1.3.2 & Meaningful Sequence \\
1.3.3 & Sensory Characteristics \\
1.3.5 & Identify Input Purpose \\
1.4.1 & Use of Color \\
1.4.3 & Contrast (Minimum) \\
1.4.4 & Resize text \\
1.4.12 & Text Spacing \\
1.4.13 & Content on Hover or Focus \\
2.1.1 & Keyboard \\
2.1.1 & Keyboard; 2.4.3 Focus Order \\
2.1.2 & No Keyboard Trap \\
2.2.1 & Timing Adjustable \\
2.4.1 & Bypass Blocks \\
2.4.2 & Page Titled \\
2.4.4 & Link Purpose (In Context); 4.1.2 Name, Role, Value \\
2.4.6 & Headings and Labels \\
2.4.7 & Focus Visible \\
2.4.7 & Focus Visible; 3.2.1 On Focus \\
2.5.3 & Label in Name \\
3.1.1 & Language of Page \\
3.2.1 & On Focus \\
3.2.2 & On Input \\
3.3.2 & Labels or Instructions \\
4.1.2 & Name, Role, Value \\
\hline
\end{tabular}


==> tables/methodology-example_report.tex <==
\begin{tabular}{|p{1.5cm}|p{6.8cm}|}
\hline
\textbf{Feature} & \textbf{Example} \\
\hline
Page title & Atlanta news, Georgia news, Breaking news from The Atlanta Journal-Constitution - AJC.com \\
\hline
Page URL & \url{https://www.ajc.com/} \\
\hline
Scan Label & scan\_1 \\
\hline
Issue ID & 2748300732 \\
\hline
Issue Type & Violation \\
\hline
Toolkit level & 1 \\
\hline
Checkpoint & 1.1.1 Non-text Content \\
\hline
WCAG level & A \\
\hline
Rule & img\_alt\_valid \\
\hline
Issue & The image has neither an accessible name nor is marked as decorative or redundant \\
\hline
Element & img \\
\hline
Code & \texttt{<img style="display: block; padding: 0px; margin: 0px; border-width: 0px; min-width: 0px; min-height: 0px; max-width: none; max-height: none; -webkit-tap-highlight-color: rgba(0, 0, 0, 0); user-select: none; box-sizing: content-box; height: 100\%; width: 100\%; top: 0px; left: 0px; position: absolute;" src="https://clipcentric-a.akamaihd.net/file/1846203/master/1720505441/RhmEzmzh?f=auto" draggable="false">} \\
\hline
\end{tabular}

